Algorithm-agnostic low-rank approximation of operator monotone matrix functions

Low-rank approximation of a matrix function, $f(A)$, is an important task in computational mathematics. Most methods require direct access to $f(A)$, which is often considerably more expensive than accessing $A$. Persson and Kressner (SIMAX 2023) avoid this issue for symmetric positive semidefinite matrices by proposing funNystr\"om, which first constructs a Nystr\"om approximation to $A$ using subspace iteration, and then uses the approximation to directly obtain a low-rank approximation for $f(A)$. They prove that the method yields a near-optimal approximation whenever $f$ is a continuous operator monotone function with $f(0) = 0$. We significantly generalize the results of Persson and Kressner beyond subspace iteration. We show that if $\widehat{A}$ is a near-optimal low-rank Nystr\"om approximation to $A$ then $f(\widehat{A})$ is a near-optimal low-rank approximation to $f(A)$, independently of how $\widehat{A}$ is computed. Further, we show sufficient conditions for a basis $Q$ to produce a near-optimal Nystr\"om approximation $\widehat{A} = AQ(Q^T AQ)^{\dagger} Q^T A$. We use these results to establish that many common low-rank approximation methods produce near-optimal Nystr\"om approximations to $A$ and therefore to $f(A)$.

==> counter-examples.tex <==
\section{Counter-Examples}

In this section, we show examples that demonstrate that the assumptions in our results in \Cref{section:black_box} are necessary. Let $\widehat{\bm{A}}$ be a symmetric rank $k$ approximation of $\bm{A}$ and define
\begin{align*}
    &\varepsilon_{\text{original}} = \frac{\|\bm{A}-\widehat{\bm{A}}\|}{\|\bm{A}-\bm{A}_{(k)}\|} - 1;\\
    &\varepsilon_{\text{function}} = \frac{\|f(\bm{A})-f(\widehat{\bm{A}})\|}{\|f(\bm{A})-f(\bm{A}_{(k)})\|} - 1;\\
\end{align*}
The results in \Cref{section:black_box} show that if $(i)$ $\bm{A} \succeq \widehat{\bm{A}}$, and $(ii)$ $f$ is a continuous operator monotone function with $f(0) = 0$, then $\varepsilon_{\text{original}} \geq \varepsilon_{\text{original}}$. One might ask if one really has to assume that $\bm{A} \succeq \widehat{\bm{A}}$ or if it is sufficient to only assume that $f$ is continous, concave, and satisfies $f(0) = 0$. We provide counter examples to show that our assumptions are necessary. More specifically, if one of the assumptions are relaxed one can have $\varepsilon_{\text{original}} \leq \varepsilon_{\text{original}}$. Table~\ref{table:assumptions} demonstrates our results.

\begin{table}[H]
\centering
\begin{tabular}{@{}lcccc@{}} \toprule
	& \multicolumn{2}{c}{Operator Monotone} & \multicolumn{2}{c}{Concave} \\ \cmidrule(lr){2-3} \cmidrule(l){4-5}
	Guarantee
		& \(\bm{A} \succeq \widehat{\bm{A}}\)
		& \(\bm{A} \cancel{\succeq} \widehat{\bm{A}}\)
		& \(\bm{A} \succeq \widehat{\bm{A}}\)
		& \(\bm{A} \cancel{\succeq} \widehat{\bm{A}}\) \\ \midrule
	Nuclear Norm
		& \(\checkmark_{\ref{theorem:nuclear_black_box}}\)
		& \(\text{\xmark}_{\ref{eg:psd-needed-for-frob-nuc}}\)
		& \(\text{\xmark}_{\ref{eg:mono-needed-for-nuc}}\)
		& \(\text{\xmark}_{\ref{eg:psd-needed-for-frob-nuc}}\) \\
	Frobenius Norm
		& \(\checkmark^*_{\ref{theorem:frobenius_black_box}}\)
		& \(\text{\xmark}_{\ref{eg:psd-needed-for-frob-nuc}}\)
		& ?
		& \(\text{\xmark}_{\ref{eg:psd-needed-for-frob-nuc}}\) \\
	Spectral Norm
		& \(\checkmark_{\ref{theorem:spectral_black_box}}\)
		& \(\checkmark_{\ref{theorem:spectral_black_box}}\)
		& ?
		& \(\text{\xmark}_{\ref{eg:mono-needed-for-spectral}}\) \\
	Singular Value
		& \(\checkmark_{\ref{theorem:eigenvalue_black_box}}\)
		& \(\checkmark_{\ref{theorem:eigenvalue_black_box}}\)
		& \(\checkmark_{\ref{theorem:eigenvalue_black_box}}\)
		& \(\checkmark_{\ref{theorem:eigenvalue_black_box}}\) \\ \bottomrule
\end{tabular}
\caption{
	Table demonstrating what guarantees exist for low-rank approximation under different assumptions.
	% We always assume \(f\) is concave with \(f(0)=0\), but do we further assume \(f\) is operator monotone?
	% We always assume the approximation \(\widehat{\bm{A}}\) is PSD, but do we further assume that \(\bm{A} \succeq \widehat{\bm{A}}\)?
	A checkmark (\checkmark) indicates that a low-rank approximation guarantee exists with the listed assumptions.
	A cross (\xmark) indicates that a counterexample with the listed assumptions violates the guarantee.
    The question marks (?) denote open problems.
	The asterisk for the Frobenius norm denotes that we make stronger assumption for that guarantee; see \Cref{section:frobenius_nuclear_black_box}.
}\label{table:assumptions}
\end{table}
We point out that we have not found a counter example for the spectral and Frobenius norm when $\bm{A} \succeq \widehat{\bm{A}}$ and $f$ is only continuous, concave, and $f(0) = 0$. 

\begin{example}[Operator Monotone is necessary for Nuclear norm]
\label{eg:mono-needed-for-nuc}
Let \(\bm{A} = \sbmat{ 1.1 \\ & 0.1 }\) and \(\widehat{\bm{A}} = \bm{v}\bm{v}^T\) where \(\bm{v}=\sbmat{1 \\ 0.095}\).
With \(k=1\) and \(f(x)=\min\{1,x\}\), we have that \(\varepsilon_{\text{function}} > 1.158\, \varepsilon_{\text{original}}\) in the Nuclear norm.
In particular, we have \(\bm{A} \succeq \widehat{\bm{A}}\), but \(f\) is not operator monotone.
\end{example}

\David{I would suggest that you pick some other values of $\delta$ and $\eta$. I also commented out the proof.} 
\begin{example}[Operator Monotone is necessary for Spectral Norm]
\label{eg:mono-needed-for-spectral}
Let \(\bm{A} = \sbmat{1+\eta \\ & \eta}\) and \(\widehat{\bm{A}} = \bm{v}\bm{v}^T\) where \(\bm{v} = \sbmat{1+\eta \\ \delta}\) for \(\eta = 10^{-8}\) and \(\delta = 10^{-10}\). 
If we take \(f(x) = \min\{1,x\}\) and \(k=1\), then we have that $\varepsilon_{\text{function}} > 1.999 \, \varepsilon_{\text{original}}$
holds in the spectral norm.
In particular, both \(f\) is not operator monotone and \(\bm{A} \cancel{\succeq} \widehat{\bm{A}}\).
\end{example}
%\begin{proof}
%We have to be careful here to avoid concerns of numerical stability, which can inflate the number here slightly.
%A commented version of the utilized matlab code is in the LaTeX source code here.
%Plug the matrices symbolically into matlab in terms of variables \(\eta\) and \(\delta\).
%Then symbolically compute the eigenvalues, and compare the epsilons as functions of \(\eta\). 
%Notably, as either \(\eta\rightarrow0\) or \(\delta\rightarrow0\), we get both \(\varepsilon_{\text{function}}\rightarrow0\) and \(\varepsilon_{\text{original}}\rightarrow0\), which is why we need both variables in the example statement.
%\end{proof}

% clear
% syms eta real;
% syms delta real;

% A = [1 + eta 0 ; 0 eta];
% v = [1 + eta; delta];
% Ahat = v*v';

% fA = [1 0 ; 0 eta];
% fAhat = simplify(v*v' / (norm(v)^2));

% eig_orig = eig(A - Ahat);
% eig_func = eig(fA - fAhat);

% eps_orig = max(abs(simplify(subs(simplify(subs(eig_orig, delta, 1e-10)), eta, 1e-8))/1e-8)) - 1;
% eps_func = max(abs(simplify(subs(simplify(subs(eig_func, delta, 1e-10)), eta, 1e-8))/1e-8)) - 1;

% Print out the epsilon values, and their ratio
% vpa(eps_orig)
% vpa(eps_func)
% vpa(eps_func / eps_orig) % > 1.999


% \begin{example}[Operator Monotone is necessary for Spectral Norm]
% \label{eg:mono-needed-for-spectral}
% Let \(\bm{A} = \sbmat{1 \\ & 0.5}\) and \(\widehat{\bm{A}} = c\bm{v}\bm{v}^T\) where \(c=\frac{1.5}{1+\eta^2}\) and \(\bm{v} = \sbmat{1 \\ \eta}\), and take \(f(x) = \min\{1,x\}\) and \(k=1\).
% Then, we have that
% \[
% 	\lim_{\eta \rightarrow 0} \frac{\varepsilon_{\text{function}}}{\varepsilon_{\text{original}}} = 1.333
% \]
% In other words, for any fixed \(\delta>0\), there exists a choice of \(\eta>0\) such that the matrices \(\bm{A}\) and \(\widehat{\bm{A}}\) have \(\varepsilon_{\text{function}} > (1.333-\delta) \varepsilon_{\text{original}}\).
% In particular, both \(f\) is not operator monotone and \(\bm{A} \cancel{\succeq} \widehat{\bm{A}}\).
% \end{example}
% \begin{proof}
% Plug the matrices symbolically into matlab, compute the eigenvalues, and compare the epsilons as functions of \(\eta\). Plot them, and observe the conclusion.
% Notably, as \(\eta\rightarrow0\), we get both \(\varepsilon_{\text{function}}\rightarrow0\) and \(\varepsilon_{\text{original}}\rightarrow0\), which is why we need this extra layer of \(\eta\) in the example statement.
% \end{proof}

\begin{example}[PSD ordering is necessary for Frobenius and Nuclear norms.]
\label{eg:psd-needed-for-frob-nuc}
Let \(\bm{A} = \sbmat{ 1 \\ & 1 \\ & & 0 }\) and \(\widehat{\bm{A}} = \bm{v}\bm{v}^T\bm{A}\bm{v}\bm{v}^T\) where \(\bm{v} = \frac1{\sqrt2}\sbmat{ 0 \\ 1 \\ 1 }\).
Then, with \(k=1\) and \(f(x) = \sqrt{x}\) we get \(\varepsilon_{\text{function}} > 1.059\varepsilon_{\text{original}}\) in the Nuclear norm and \(\varepsilon_{\text{function}} > 1.036\varepsilon_{\text{original}}\) in the Frobenius norm.
In particular, \(f\) is operator monotone, but \(\bm{A}\cancel{\succeq}\widehat{\bm{A}}\).
\end{example}



==> doc.tex <==

\Chris{May 23, 2023: Can we update these to reflex what we were able to show? I.e. did the last approach work out and what were we able to prove?}

\David{23 May 2023: Updated. Currently this document is in a bit of disarray, but I'll start cleaning it up these coming days. }
\begin{itemize}
    \item Have: nice complete analysis of Nystrom as the postprocessing step for Krylov iteration. We currently have spectral, nuclear, Frobenius and per vector error. We still need to type up some things: 3 properties from MM15 (running block Krylov on inverse function), Frobenius norm, clean up this document. 
    \item Have not checked yet: Using a block size of $2k$ and prove Frobenius norm from the per vector guarantee. Does it work for all Schatten norms?
    %\begin{itemize}
        %\item We *would* have this if we new the standard block Krylov method was optimal in 4-norm.
        %\item We can probably prove this directly using David's per vector guarantees if we are willing to use block size $2k$.  Would need to combine with a gap-dependent rate.
        %\item Actually, if we are willing to use block size $2k$, can we get all Schatten norms?
    %\end{itemize}
    \item What's the benefit of Nystrom? It's strictly better than two and one-sided projection for PSD matrices. Doesn't require the extra mat-vec that one sided projection. 
    %\item Alternative approach to analyzing error of funNystrom is just to view it as running block Krylov on powers of $f^{-1}(A)$. Let's see if this works! \David{See Lemma~\ref{lemma:krylov_inverse} for a start of this approach.}
    \item Other things we have: How to go from one sided to two sided projections for a $(1+\varepsilon)$ LRA. 
\end{itemize}

\section{Introduction}
\subsection{Notation}
We consider a symmetric positive semidefinite (SPSD) matrix $\bm{A}$ with eigenvalue decomposition
\begin{equation*}
    \bm{A} = \bm{U} \bm{\Lambda} \bm{U}^T = \begin{bmatrix} \bm{U}_1 & \bm{U}_2 \end{bmatrix} \begin{bmatrix} \bm{\Lambda}_1 & \\ & \bm{\Lambda}_2 \end{bmatrix} \begin{bmatrix} \bm{U}_1^T \\ \bm{U}_2^T \end{bmatrix},
\end{equation*}
where $\bm{\Lambda}_1 \in \mathbb{R}^{k \times k}$ contains the $k$ largest eigenvalues and $\bm{U}_1 \in \mathbb{R}^{n \times k}$ the corresponding eigenvectors. For a matrix $\bm{B}$ we denote by $\bm{P}_{\bm{B}}$ the orthogonal projector onto $\range(\bm{B})$. Hence, if $\bm{V}$ is an orthonormal basis for $\range(\bm{B})$ we have $\bm{P}_{\bm{B}} = \bm{V} \bm{V}^T$. Let let $\bm{\Omega} \in \mathbb{R}^{n \times k}$ denote a sketching matrix and we define $\bm{\Omega}_i = \bm{U}_i^T \bm{\Omega}$ for $i = 1,2$. We assume that $\bm{\Omega}_1$ has full rank. For a matrix $\bm{B}$ we denote by $\bm{B}_k$ a best rank $k$ approximation of $\bm{B}$ obtained by truncating the singular value decomposition. 

\section{A generalization to Krylov subspaces}
\begin{theorem}\label{theorem:krylov_generalization}
    Let $g:[0,\infty) \mapsto [0,\infty)$ be a continuous and increasing function so that $g(0)=0$ and define
    \begin{align*}
        &x^* = \sup\left\{x \in [0,\infty]:g(x) \leq (1+\gamma)g(\lambda_{k+1})\right\};\\
        &x_* = \sup\left\{x \in [0,\lambda_{k}]: g(x) \leq \frac{g(\lambda_k)}{1+\gamma}\right\}
    \end{align*}
    Let $p_1 = p_1^{(q,\gamma)}, p_2 = p_2^{(q,\gamma)}:[0,\infty) \mapsto [0,\infty)$ be functions, parametrized by $q \in \mathbb{N}$ and $\gamma \in (0,1]$, so that
    \begin{align}
    &p_1(x) \geq g(x) \text{ for } x \geq x^*;\\
    &p_2(x) \geq g(x) \text{ for } x \geq \lambda_{k};\\
    &|p_1(x)|^2 \leq \delta^{(q,\gamma)} g(\lambda_{k+1})^2 \text{ for } x \in [0,\lambda_{k+1}];\\
    &|p_2(x)|^2 \leq \frac{\delta^{(q,\gamma)} g(\lambda_k)^2}{(1+\gamma)^2} \text{ for } x \in \left[0, x_*\right]. 
    \end{align}
    Let $\bm{Y}_1$ and $\bm{Y}_2$ be orthonormal bases for $\range(p_1(\bm{A}) \bm{\Omega})$ and $\range(p_2(\bm{A}) \bm{\Omega})$ respectively, and assume that $\bm{Q}$ is an orthonormal basis so that
    \begin{equation*}
        \range(\bm{Y}_1), \range(\bm{Y}_2) \subseteq \range(\bm{Q}). 
    \end{equation*}
    Assume without loss of generality that $\bm{Q}$ is chosen so that $\bm{Q}_{:,1:\ell} \bm{Q}_{:,1:\ell}^T g(\bm{A}) = (\bm{Q} \bm{Q}^T g(\bm{A}))_{\ell}$. 

    Let $m$ be the number of singular values so that $(1+\gamma) g(\lambda_{k+1}) \leq g(\lambda_i)$, and let $w$ be the number of singular values so that $\frac{1}{1+\gamma}g(\lambda_k) \leq g(\lambda_i) < g(\lambda_k)$. Let
    \begin{equation*}
        \varepsilon\geq n(1+\|\bm{\Omega}_2\bm{\Omega}_1^{-1}\|_2^2) \delta^{(q,\gamma)}
    \end{equation*}
    and assume $\varepsilon < 1.$ Then, for $\gamma = \varepsilon$ or $\gamma = \min\left\{1, \frac{g(\lambda_k) - g(\lambda_{k+1})}{g(\lambda_k)}\right\}$
    \begin{itemize}
        \item[1.] For all $\ell \leq m$ we have $\|g(\bm{A}) - \bm{Q}_{:,1:\ell}\bm{Q}_{:,1:\ell}^T g(\bm{A})\|_F^2 \leq \|g(\bm{A}) - g(\bm{A})_{\ell}\|_F^2 + \varepsilon g(\lambda_{k+1})^2$,
    \end{itemize}
    and for $\gamma = \varepsilon$ we have
    \begin{itemize}
        \item[2.] for all $\ell \leq k$ we have $g(\lambda_{\ell})^2 - \sigma_{\ell}(\bm{Q}\bm{Q}^T g(\bm{A}))^2 \leq 4\varepsilon g(\lambda_{k+1})^2$;
        \item[3.] for all $\ell \leq k$ we have $\|g(\bm{A}) - \bm{Q}_{:,1:\ell}\bm{Q}_{:,1:\ell}^T g(\bm{A})\|_F^2 \leq \|g(\bm{A}) - g(\bm{A})_{\ell}\|_F^2 + 6(w+1)\varepsilon g(\lambda_{k+1})^2$.
    \end{itemize}
\end{theorem}
The proof is identical to the proofs of \cite[Lemma 9]{MM15}. For completeness, we include the proof in Appendix~\ref{appendix:krylov_generalization}. 

As corollaries of Theorem~\ref{theorem:krylov_generalization} we have spectral and Frobenius norm guarantees and eigenvalue guarantees. 
\begin{theorem}\label{theorem:main_results}
Consider the setting of Theorem~\ref{theorem:krylov_generalization}. Then, for $\gamma = \varepsilon$ or $\gamma = \min\left\{1,\frac{g(\lambda_k) - g(\lambda_{k+1})}{g(\lambda_{k+1})}\right\}$ we have
\begin{itemize}
    \item[1.] $\|g(\bm{A})-\bm{Q}_{:,1:k}\bm{Q}_{:,1:k}^T g(\bm{A})\|_2^2 \leq (1+2\varepsilon) g(\lambda_{k+1})^2$,
\end{itemize}
and for $\gamma = \varepsilon$ we have
\begin{itemize}
    \item[2.] for all $\ell \leq k$ we have $g(\lambda_{\ell})^2 - \sigma_{\ell}(\bm{Q}\bm{Q}^T g(\bm{A}))^2 \leq 4\varepsilon g(\lambda_{k+1})^2$;
    \item[3.] $\|g(\bm{A}) - \bm{Q}_{:,1:k}\bm{Q}_{:,1:k}^T g(\bm{A})\|_F^2 \leq (1+30\varepsilon)\|g(\bm{A}) - g(\bm{A})_{k}\|_F^2$.
\end{itemize}
\end{theorem}
The proof is identical to \cite[Theorems 10-12]{MM15}. For completeness, we include the proof in Appendix~\ref{appendix:krylov_generalization}. 

The next lemma is a generalization of \cite[Lemma 5]{MM15}. 

\begin{lemma}\label{lemma:polynomial2}
Let $f:[0,\infty) \mapsto [0,\infty)$ be continuously differentiable and concave function and satisfy $f(0) = 0$. Let $h:[0,\infty) \mapsto [0,\infty)$ be an arbitrary increasing function so that $h(x) > 0$ for $x > 0$. For a given pair $\alpha > 0$ and $\gamma \in (0,1]$ define
\begin{equation*}
    x^* = \sup\limits \left\{x \in [0,\infty] : f(x) \leq (1+\gamma)f(\alpha) \right\}.
\end{equation*}
Let $T_q$ be the $q^{\text{th}}$ degree Chebyshev polynomial. Define, 
\begin{equation*}
    \widetilde{p}_{q,\alpha,\gamma,f,h}(x) = \frac{(1+\gamma)f(\alpha) h(x)T_{q}(x/\alpha)}{h(\alpha)T_q(x^*/\alpha)}.
\end{equation*}
Then $\widetilde{p} = \widetilde{p}_{q,\alpha,\gamma,f,h}$ satisfies
\begin{enumerate}
    \item[(i)] $\widetilde{p}(x) \geq f(x)$ for $x \geq x^*$;
    \item[(ii)] $|\widetilde{p}(x)| \leq \frac{2(1+\gamma)f(\alpha)}{2^{q\sqrt{\gamma}}}$ for $x \in [0,\alpha]$. 
\end{enumerate}
%Furthermore, if $q$ is odd (even) then $p$ contains only odd (even) degree monomials. In addition, the same bounds hold for the function
%\begin{equation*}
    %\widetilde{p}_{q,\alpha,\gamma}(x) = \sqrt{\frac{x}{\alpha}} p_{q,\alpha,\gamma,f}(x).
%\end{equation*}
\end{lemma}
\begin{proof}
First consider the case when $x^* = \infty$. Then, $(i)$ becomes irrelevant and $(ii)$ trivially holds, since $\lim\limits_{x \rightarrow \infty} T_q(x) = +\infty$. 
\David{Note to self: In fact we should remove this case analysis and just immediately assume that $x^* < \infty$. We never use the Lemma when $x^* = \infty$.}\Raph{Note to self: this is the case when \(m=0\) in MM15. It's trivially because if \(x^* = \infty\) then that means that no matter how large a singular value of \(\mathbf A\) is, we cannot guarantee it's in the easy-to-converge-to directions. That's what \(m=0\) means. So... who cares if it's a trivial polynomial \(\tilde p(x) = 0 ~ \forall x\).}

Now assume that $x^* < +\infty$. Since $f$ is continous we have $f(x^*) = (1+\gamma)f(\alpha)$. First note that $x^* > \alpha$ since $f$ is increasing and $f(x^*) = (1+\gamma)f(\alpha) > f(\alpha)$. Hence, there exists some $\eta > 0$ so that $x^* = (1+\eta)\alpha$. Thus, we can write
\begin{equation*}
    \widetilde{p}(x) = \frac{f((1+\eta)\alpha) h(x) T_q(x/\alpha)}{h(\alpha)T_q(1+\eta)}
\end{equation*}
Since $h(x)/h(\alpha) \geq 1$ for $x \geq (1+\eta)\alpha$ and $h(x)/h(\alpha) \leq 1$ for $x \in [0,\alpha]$, it suffices to show that the polynomial
\begin{equation*}
    p(x) = \frac{f((1+\eta)\alpha) T_q(x/\alpha)}{T_q(1+\eta)}
\end{equation*}
satisfies the bounds in the statement. 

Note that
\begin{equation*}
    p(x^*) = f(x^*).
\end{equation*}
Hence, to show $(i)$ we only need to show 
\begin{equation}\label{eq:derivative_inequality4}
    p'(x) \geq f'(x) \quad \text{for } x \geq (1+\eta)\alpha. 
\end{equation}
Note that $T_q$ is convex, increasing, and positive on $[(1+\eta)\alpha,\infty)$. Hence, the smallest value of $p'(x)$ on $[(1+\eta)\alpha,\infty)$ is attained at $x = (1+\eta)\alpha$. Furthermore, since $f$ is concave, increasing, and positive on $[(1+\eta)\alpha,\infty)$ the largest value of $f'(x)$ on $[(1+\eta)\alpha,\infty)$ is attained at $x = (1+\eta)\alpha$. Hence, to show \eqref{eq:derivative_inequality4} we only need to show
\begin{equation}\label{eq:derivative_inequality5}
    p'((1+\eta)\alpha) \geq f'((1+\eta)\alpha).
\end{equation}
We have
\begin{equation*}
    p'(x) = \frac{f((1+\eta)\alpha) T_{q}'(x/\alpha)}{\alpha T_q(1+\eta)} = \frac{(1+\eta)T_{q}'(x/\alpha)}{T_q(1+\eta)} \frac{f((1+\eta)\alpha)}{(1+\eta)\alpha}.
\end{equation*}
Hence, to show \eqref{eq:derivative_inequality5} is equivalent to show
\begin{equation*}
    \frac{(1+\eta)T_{q}'(x/\alpha)}{T_q(1+\eta)} \geq \frac{(1+\eta)\alpha f'((1+\eta)\alpha)}{f((1+\eta)\alpha)}.
\end{equation*}
Contained in the proof of \cite[Lemma 5]{MM15} it was shown that for $x \geq (1+\gamma)\alpha$
\begin{equation*}
    \frac{(1+\gamma)T_{q}'(x/\alpha)}{T_q(1+\gamma)} \geq 1.
\end{equation*}
Hence, for any $y > 0$ it suffices to show
\begin{equation}\label{eq:derivative_inequality6}
    \frac{yf'(y)}{f(y)} \leq 1.
\end{equation}
Since $f$ is concave and continuously differentiable we know that for any $y,z \geq 0$ we have $f(z) \leq f(y) + f'(y)(z-y)$. By setting $z = 0$ and using $f(0) = 0$ we obtain $0 \leq f(y) - yf'(y)$, which is equivalent to \eqref{eq:derivative_inequality6}, and thus yields $(i)$. 

To show $(ii)$ we use that $|T(x/\alpha)| \leq 1$ for $x \in [0,\alpha]$ to get
\begin{equation*}
    |p(x)| \leq \frac{(1+\gamma)f(\alpha)}{T_{q}(1+\eta)}.
\end{equation*}
Contained in the proof of \cite[Lemma 5]{MM15} it was shown that $\frac{1}{T_{q}(1+\eta)} \leq \frac{2}{2^{q\sqrt{\eta}}}$. Hence, to show $(ii)$ we only need to show that $\eta \geq \gamma$. By concavity of $f$ we have
\begin{equation*}
    f((1+\eta) \alpha) = (1+\gamma) f(\alpha) \geq f((1+\gamma) \alpha).
\end{equation*}
If $(1+\gamma)\alpha > (1+\eta)\alpha = x^*$ we must have $(1+\gamma) f(\alpha) = f((1+\gamma) \alpha)$ with $(1+\gamma)\alpha > x^*$, which contradicts the definition of $x^*$. So we must have $\gamma \leq \eta$, as required.

%The penultimate statement follows from the fact that odd (even) degree Chebyshev polynomials contain only odd (even) degree monomials. The final statement is a consequence of $\sqrt{\frac{x}{\alpha}} \geq 1$ for $x \geq (1+\gamma)\alpha$ and $\sqrt{\frac{x}{\alpha}} \leq 1$ for $x \in [0,\alpha]$.
\end{proof}

The following lemma will be useful for when we analyze subspace iteration.

\begin{lemma}\label{lemma:polynomial3}
Consider the setting of Lemma~\ref{lemma:polynomial2}. Define, 
\begin{equation*}
    \widehat{p}_{q,\alpha,\gamma,f,h}(x) = \frac{(1+\gamma)f(\alpha) h(x)(x/\alpha)^q}{h(\alpha)(x^*/\alpha)^q}.
\end{equation*}
Then $\widetilde{p} = \widetilde{p}_{q,\alpha,\gamma,f,h}$ satisfies
\begin{enumerate}
    \item[(i)] $\widehat{p}(x) \geq f(x)$ for $x \geq x^*$;
    \item[(ii)] $|\widehat{p}(x)| \leq \frac{(1+\gamma)f(\alpha)}{2^{q\gamma}}$ for $x \in [0,\alpha]$. 
\end{enumerate}
%Furthermore, if $q$ is odd (even) then $p$ contains only odd (even) degree monomials. In addition, the same bounds hold for the function
%\begin{equation*}
    %\widetilde{p}_{q,\alpha,\gamma}(x) = \sqrt{\frac{x}{\alpha}} p_{q,\alpha,\gamma,f}(x).
%\end{equation*}
\end{lemma}
The proof is identical to Lemma~\ref{lemma:polynomial2}.\footnote{We use that $\frac{1}{(1+\gamma)^{q}} \leq \frac{1}{2^{q\gamma}}$}

\begin{remark}
    For $(ii)$ in Lemma~\ref{lemma:polynomial2} and Lemma~\ref{lemma:polynomial3} we can replace $\gamma$ in the denominator with $\eta$. 
\end{remark}

\section{Error bounds}
\begin{theorem}
    Let
    \begin{equation*}
        q \geq \frac{\log_2\left(\frac{4n(1+\varepsilon)^2}{\varepsilon}(1+\|\bm{\Omega}_2 \bm{\Omega}_1^{-1}\|_2^2)\right)}{2\sqrt{\varepsilon}}.
    \end{equation*}
    and let $\bm{Q}$ be an orthonormal basis for $\range\left(\begin{bmatrix} \bm{\Omega} & \bm{A}\bm{\Omega} & \cdots &\bm{A}^q \bm{\Omega} \end{bmatrix} \right)$.  Let 
    \begin{equation*}
        \widehat{\bm{A}} = \bm{A}\bm{Q}(\bm{Q}^T \bm{A} \bm{Q})^{\dagger} \bm{Q}^T \bm{A},
    \end{equation*}
    denote the Nyström approximation of $\bm{A}$. Then, for any operator monotone function $f$ satisfying $f(0) = 0$ we have
    \begin{equation*}
        \|f(\bm{A}) - f(\widehat{\bm{A}}_k)\|_2 \leq (1+2\varepsilon) f(\lambda_{k+1}).
    \end{equation*}
\end{theorem}
\begin{proof}
Note that 
\begin{equation*}
    \widehat{\bm{A}} = (\bm{P}_{\bm{A}^{1/2} \bm{Q}}\bm{A}^{1/2})^T (\bm{P}_{\bm{A}^{1/2} \bm{Q}}\bm{A}^{1/2}), \quad \widehat{\bm{A}}_k = (\bm{P}_{\bm{A}^{1/2} \bm{Q}}\bm{A}^{1/2})^T_k (\bm{P}_{\bm{A}^{1/2} \bm{Q}}\bm{A}^{1/2})_k. 
\end{equation*}
Let $\bm{W}$ be an orthonormal basis for $\range(\bm{A}^{1/2} \bm{Q})$ chosen so that
\begin{equation*}
    \bm{W}_{:,1:k} \bm{W}_{:,1:k}^T \bm{A}^{1/2} = (\bm{W}\bm{W}^T \bm{A}^{1/2})_k.
\end{equation*}
Then,
\begin{equation*}
    \|\bm{A} - \widehat{\bm{A}}_k\|_2^2 = \|(\bm{I} - \bm{W}_{:,1:k} \bm{W}_{:,1:k}^T) \bm{A}^{1/2}\|_2^2.
\end{equation*}
Now define $p_1 =\widetilde{p}_{q,\lambda_{k+1},\varepsilon,f,\sqrt{x}}$ from Lemma~\ref{lemma:polynomial3}. 
\end{proof}

\section{Error bounds}
\subsection{Spectral norm error bounds}
\begin{theorem}
    Let $\bm{Q}$ be an orthonormal basis for 
    \begin{equation*}
        \range\left(\begin{bmatrix} \bm{\Omega} & \bm{A}\bm{\Omega} & \cdots &\bm{A}^q \bm{\Omega} \end{bmatrix} \right),
    \end{equation*}
    where
    \begin{equation*}
        q \geq \frac{\log_2\left(\frac{4n(1+\varepsilon)^2}{\varepsilon}(1+\|\bm{\Omega}_2 \bm{\Omega}_1^{-1}\|_2^2)\right)}{2\sqrt{\varepsilon}}.
    \end{equation*}
    Let 
    \begin{equation*}
        \widehat{\bm{A}} = \bm{A}\bm{Q}(\bm{Q}^T \bm{A} \bm{Q})^{\dagger} \bm{Q}^T \bm{A},
    \end{equation*}
    denote the Nyström approximation of $\bm{A}$. Then, for any operator monotone function $f$ satisfying $f(0) = 0$ we have
    \begin{equation*}
        \|f(\bm{A}) - f(\widehat{\bm{A}}_k)\|_2 \leq (1+2\varepsilon) f(\lambda_{k+1}).
    \end{equation*}
\end{theorem}
\begin{proof}
Note that
\begin{equation*}
    \widehat{\bm{A}} = \bm{A}^{1/2} \bm{P}_{\bm{A}^{1/2} \bm{Q}}\bm{A}^{1/2} = (\bm{P}_{\bm{A}^{1/2} \bm{Q}}\bm{A}^{1/2})^T (\bm{P}_{\bm{A}^{1/2} \bm{Q}}\bm{A}^{1/2}).
\end{equation*}
Let $\widehat{\bm{P}}^{(k)}$ be the orthogonal projection so that $\widehat{\bm{P}}^{(k)} \bm{A}^{1/2} = \widehat{\bm{P}}^{(k)}\bm{P}_{\bm{A}^{1/2} \bm{Q}}\bm{A}^{1/2} = (\bm{P}_{\bm{A}^{1/2} \bm{Q}}\bm{A}^{1/2})_k$, where we used $\range(\widehat{\bm{P}}_k) \subseteq \range(\bm{P}_{\bm{A}^{1/2} \bm{Q}})$. Hence, we have 
\begin{equation*}
    \widehat{\bm{A}}_k = (\bm{P}_{\bm{A}^{1/2} \bm{Q}}\bm{A}^{1/2})_k^T (\bm{P}_{\bm{A}^{1/2} \bm{Q}}\bm{A}^{1/2})_k = \bm{A}^{1/2} \widehat{\bm{P}}^{(k)}\bm{A}^{1/2}. 
\end{equation*}
Consequently, 
\begin{equation*}
    \|\bm{A}-\widehat{\bm{A}}_k\|_{2} = \|\bm{A}^{1/2}(\bm{I}-\widehat{\bm{P}}^{(k)})\bm{A}^{1/2}\|_{2} = \|(\bm{I}-\widehat{\bm{P}}^{(k)})\bm{A}^{1/2}\|_{2}^2 = \|\bm{A}^{1/2} - (\bm{P}_{\bm{A}^{1/2} \bm{Q}} \bm{A}^{1/2})_k\|_{2}^2.
\end{equation*}

     Applying Lemma~\ref{lemma:property1} to $g(x) = \sqrt{x}$ gives
    \begin{equation*}
        \|\bm{A}^{1/2} - (\bm{P}_{\bm{A}^{1/2} \bm{Q}} \bm{A}^{1/2})_m\|_{F}^2 \leq \|\bm{A}^{1/2} - \bm{A}_m^{1/2}\|_F^2 + \varepsilon \lambda_{k+1}.
    \end{equation*}
    By \cite[Theorem 3.4]{gu_subspace} we have
    \begin{equation*}
        \|\bm{A}^{1/2} - (\bm{P}_{\bm{A}^{1/2} \bm{Q}} \bm{A}^{1/2})_m\|_{2}^2 \leq \lambda_{m+1} + \varepsilon \lambda_{k+1} \leq (1+2\varepsilon) \lambda_{k+1}.
    \end{equation*}
    Now note that $\bm{A} \succeq \widehat{\bm{A}} \succeq \widehat{\bm{A}}_k \succeq \bm{A}_m \succeq \bm{0}$. Hence, by \cite[Lemma 3.1 (i)]{persson2022randomized} and Lemma~\ref{lemma:nystrom_truncation} we have
    \begin{align*}
        \|\bm{A}-\widehat{\bm{A}}_k\|_2 \leq \|\bm{A}-\widehat{\bm{A}}_m\|_2  = \|\bm{A}^{1/2} - (\bm{P}_{\bm{A}^{1/2} \bm{Q}} \bm{A}^{1/2})_m\|_{2}^2 \leq (1+2\varepsilon) \lambda_{k+1}.
    \end{align*}
    By \cite[Theorem 1]{ando} we have
    \begin{equation*}
        \|f(\bm{A}) - f(\widehat{\bm{A}}_k)\|_2 \leq \|f(\bm{A} - \widehat{\bm{A}}_k)\|_2 = f(\|\bm{A} - \widehat{\bm{A}}_k\|_2) \leq f((1+2\varepsilon)\lambda_{k+1}) \leq (1+2\varepsilon) f(\lambda_{k+1}),
    \end{equation*}
    as required.
\end{proof}








\section{Generalizing bounds}
\subsection{General results}
\David{Maybe insert some general properties of concave functions here. Also some statements involving the regularity of operator monotone functions.}

\David{Maybe we should say that the bounds below hold for all $x \geq x^*$ where $f(x^*) = (1+\gamma)f(\alpha)$ and for $x \in [0,\alpha]$. This would avoid using properties of concave functions and we could probably completely black-box the analysis from \cite{MM15}. It would also avoid any issues of $f$ not being strictly increasing. }
\begin{lemma}\label{lemma:polynomial}
For any $\alpha \geq 0$ and $\gamma \in (0,1]$ we define
\begin{equation*}
    \widetilde{p}_{q,\alpha,\gamma,f}(x) = \frac{f((1+\gamma)\alpha) \sqrt{x/\alpha}T_{q}(x/\alpha)}{T_q(1+\gamma)}.
\end{equation*}
Then $\widetilde{p} = \widetilde{p}_{q,\alpha,\gamma,f}$ satisfies
\begin{enumerate}
    \item[(i)] $\widetilde{p}(x) \geq f(x)$ for $x \geq (1+\gamma)\alpha$;
    \item[(ii)] $|\widetilde{p}(x)| \leq \frac{2f((1+\gamma)\alpha)}{2^{q\sqrt{\gamma}}}$ for $x \in [0,\alpha]$. 
\end{enumerate}
%Furthermore, if $q$ is odd (even) then $p$ contains only odd (even) degree monomials. In addition, the same bounds hold for the function
%\begin{equation*}
    %\widetilde{p}_{q,\alpha,\gamma}(x) = \sqrt{\frac{x}{\alpha}} p_{q,\alpha,\gamma,f}(x).
%\end{equation*}
\end{lemma}
\begin{proof}
Since $\sqrt{\frac{x}{\alpha}} \geq 1$ for $x \geq (1+\gamma)\alpha$ and $\sqrt{\frac{x}{\alpha}} \leq 1$ for $x \in [0,\alpha]$, it suffices to show that the polynomial
\begin{equation*}
    p(x) = \frac{f((1+\gamma)\alpha)T_{q}(x/\alpha)}{T_q(1+\gamma)}
\end{equation*}
satisfies the bounds in the statement. Note that
\begin{equation*}
    p((1+\gamma)\alpha) = f((1+\gamma)\alpha).
\end{equation*}
Hence, to show $(i)$ we only need to show 
\begin{equation}\label{eq:derivative_inequality}
    p'(x) \geq f'(x) \quad \text{for } x \geq (1+\gamma)\alpha. 
\end{equation}
Note that $T_q$ is convex, increasing, and positive on $[(1+\gamma)\alpha,\infty)$. Hence, the smallest value of $p'(x)$ on $[(1+\gamma)\alpha,\infty)$ is attained at $x = (1+\gamma)\alpha$. Furthermore, since $f$ is concave, increasing, and positive on $[(1+\gamma)\alpha,\infty)$ the largest value of $f'(x)$ on $[(1+\gamma)\alpha,\infty)$ is attained at $x = (1+\gamma)\alpha$. Hence, to show \eqref{eq:derivative_inequality} we only need to show
\begin{equation}\label{eq:derivative_inequality2}
    p'((1+\gamma)\alpha) \geq f'((1+\gamma)\alpha).
\end{equation}
We have
\begin{equation*}
    p'(x) = \frac{f((1+\gamma)\alpha) T_{q}'(x/\alpha)}{\alpha T_q(1+\gamma)} = \frac{(1+\gamma)T_{q}'(x/\alpha)}{T_q(1+\gamma)} \frac{f((1+\gamma)\alpha)}{(1+\gamma)\alpha}.
\end{equation*}
Hence, to show \eqref{eq:derivative_inequality2} is equivalent to show
\begin{equation*}
    \frac{(1+\gamma)T_{q}'(x/\alpha)}{T_q(1+\gamma)} \geq \frac{(1+\gamma)\alpha f'((1+\gamma)\alpha)}{f((1+\gamma)\alpha)}.
\end{equation*}
Contained in the proof of \cite[Lemma 5]{MM15} it was shown that 
\begin{equation*}
    \frac{(1+\gamma)T_{q}'(x/\alpha)}{T_q(1+\gamma)} \geq 1.
\end{equation*}
Hence, for any $y > 0$ it suffices to show
\begin{equation}\label{eq:derivative_inequality3}
    \frac{yf'(y)}{f(y)} \leq 1.
\end{equation}
Since $f$ is concave we know that for any $y,z \geq 0$ we have $f(z) \leq f(y) + f'(y)(z-y)$. By setting $z = 0$ and using $f(0) = 0$ we obtain $0 \leq f(y) - yf'(y)$, which is equivalent to \eqref{eq:derivative_inequality3}, and thus yields $(i)$. 

To show $(ii)$ we use that $|T(x/\alpha)| \leq 1$ for $x \in [0,\alpha]$ to get
\begin{equation*}
    |p(x)| \leq \frac{f((1+\gamma)\alpha)}{T_{q}(1+\gamma)}.
\end{equation*}
Contained in the proof of \cite[Lemma 5]{MM15} it was shown that $\frac{1}{T_{q}(1+\gamma)} \leq \frac{2}{2^{q\sqrt{\gamma}}}$, which yields $(ii)$. 

%The penultimate statement follows from the fact that odd (even) degree Chebyshev polynomials contain only odd (even) degree monomials. The final statement is a consequence of $\sqrt{\frac{x}{\alpha}} \geq 1$ for $x \geq (1+\gamma)\alpha$ and $\sqrt{\frac{x}{\alpha}} \leq 1$ for $x \in [0,\alpha]$.
\end{proof}
\begin{lemma}[{\cite[Theorem 9.1]{rsvd}}]\label{lemma:structural}
Let $\bm{Y} = \bm{A} \bm{\Omega}$, and assume that $\bm{\Omega}_1$ is full rank. Then,
\begin{equation*}
    \|(\bm{I} - \bm{P}_{\bm{Y}})\bm{A}\|_F^2 \leq (1+\|\bm{\Omega}_2\bm{\Omega}_1^{-1}\|_2^2)\|\bm{\Lambda}_2\|_F^2.
\end{equation*}
\end{lemma}
\begin{lemma}[{\cite[Lemma 14]{woodruff_sketching}}]\label{lemma:constrained_best_low_rank_approximation}
    Given an orthonormal basis $\bm{Q} \in \mathbb{R}^{n \times \ell}$. Then, 
    \begin{equation*}
        \|\bm{A} - (\bm{Q}\bm{Q}^T\bm{A})_k\|_F = \min\limits_{\bm{C}: \rank(\bm{C})\leq k}\|\bm{A} - \bm{Q}\bm{C}\|_F.
    \end{equation*}
\end{lemma}
\subsection{Operator norm guarantees}
\begin{lemma}\label{lemma:property1}
    Suppose that $\bm{Q}$ is an orthonormal basis for
    \begin{equation*}
        \range\left( \begin{bmatrix} \bm{\Omega} & \bm{A} \bm{\Omega} & \cdots & \bm{A}^{q} \bm{\Omega} \end{bmatrix}\right),
    \end{equation*}
    where we choose $q$ so that
    \begin{equation*}
        q \geq \frac{\log_2\left(\frac{4n(1+\varepsilon)^2}{\varepsilon}(1+\|\bm{\Omega}_2 \bm{\Omega}_1^{-1}\|_2^2)\right)}{2\sqrt{\varepsilon}}.
    \end{equation*}
   Furthermore, let $m$ denote the number of singular values of $\bm{A}$ so that $\lambda_i \leq (1+\varepsilon) \lambda_{k+1}$. Then, for any operator monotone function $g$ satisfying $g(0) = 0$ we have for all $\ell \leq m$
    \begin{equation*}
        \|g(\bm{A})-(\bm{P}_{\bm{A}^{1/2}\bm{Q}}g(\bm{A}))_{\ell}\|_F^2 \leq \varepsilon g(\lambda_{k+1})^2 + \|g(\bm{A})-g(\bm{A}_{\ell})\|_F^2.
    \end{equation*}
\end{lemma}
\begin{proof}
\David{The proof is identical to \cite[Lemma 9, Property 1]{MM15}. I have typed it out just to make sure that everything works out.}Let $\widetilde{p} = \widetilde{p}_{q,\sigma_{k+1},\varepsilon,g}$ from Lemma~\ref{lemma:polynomial}. Let $\bm{V}$ be an orthonormal basis for $\range(\widetilde{p}(\bm{A}) \bm{\Omega})$. By Lemma~\ref{lemma:structural} and the fact that $\|\widetilde{p}(\bm{\Sigma}_2)\|_F$ is the best rank $k$ approximation Frobenius norm error of $\widetilde{p}(\bm{A})$ we have 
\begin{equation*}
    \|(\bm{I}-\bm{V}\bm{V}^T)\widetilde{p}(\bm{A})\|_F^2 \leq (1+\|\bm{\Omega}_2\bm{\Omega}_1^{-1}\|_2^2) \|\widetilde{p}(\bm{\Lambda}_2)\|_F^2.
\end{equation*}
By Lemma~\ref{lemma:polynomial} and using that $g(tx) \leq tg(x)$ for $t \geq 1$,\footnote{To show this define $h_t(x) = \frac{g(tx)}{t}$. Note that $h_1(x) = g(x)$ and $h_t(0) = g(0) = 0$. Now it suffices to show that $h'_t(x) \leq g'(x)$. Note that $h'_t(x) = g'(tx) \leq g'(x)$, since $g'$ is a decreasing function, a consequence of concavity.} a consequence of the concavity of $g$ \David{we crucially use concavity here}, we have
\begin{align*}
    &(1+\|\bm{\Omega}_2\bm{\Omega}_1^{-1}\|_2^2) \|\widetilde{p}(\bm{\Sigma}_2)\|_F^2 \leq \frac{4n}{2^{2\sqrt{\varepsilon}q}}(1+\|\bm{\Omega}_2\bm{\Omega}_1^{-1}\|_2^2) g((1+\varepsilon)\lambda_{k+1})^2 \leq \\
    & \frac{4n(1+\varepsilon)^2}{2^{2\sqrt{\varepsilon}q}}(1+\|\bm{\Omega}_2\bm{\Omega}_1^{-1}\|_2^2) g(\lambda_{k+1})^2 \leq \varepsilon g(\lambda_{k+1})^2.
\end{align*}
Hence, to show the claim it suffices to show that
\begin{equation}\label{eq:low_rank_difference}
     \|(\bm{I}-\bm{V}\bm{V}^T)\widetilde{p}(\bm{A})\|_F^2 \geq \|g(\bm{A})-(\bm{P}_{\bm{A}^{1/2}\bm{Q}}g(\bm{A}))_{\ell}\|_F^2 - \|g(\bm{A})-g(\bm{A}_{\ell})\|_F^2.
\end{equation}
For any $\ell \leq m$, by Lemma~\ref{lemma:polynomial} and that $\widetilde{p}(\bm{A})$ and $g(\bm{A}_{\ell})$ commute we have
\begin{equation*}
    \widetilde{p}(\bm{A})^2 \succeq g(\bm{A}_{\ell})^2.
\end{equation*}
Consequently,
\begin{align*}
    &\|(\bm{I}-\bm{V}\bm{V}^T)\widetilde{p}(\bm{A})\|_F^2 = \tr((\bm{I}-\bm{V}\bm{V}^T)\widetilde{p}(\bm{A})^2 (\bm{I}-\bm{V}\bm{V}^T)) \geq \\
    &\tr((\bm{I}-\bm{V}\bm{V}^T)g(\bm{A}_{\ell})^2 (\bm{I}-\bm{V}\bm{V}^T)) = \|(\bm{I}-\bm{V}\bm{V}^T)g(\bm{A}_{\ell})\|_F^2 = \\
    & \|g(\bm{A})-\bm{V}\bm{V}^Tg(\bm{A}_{\ell})\|_F^2 - \|g(\bm{A})-g(\bm{A}_{\ell})\|_F^2.
\end{align*}
Note that $\range(\bm{V}) \subseteq \range(\bm{A}^{1/2}\bm{Q})$, so $\bm{V}\bm{V}^T g(\bm{A}_{\ell})$ is a rank $\ell$ approximation of $g(\bm{A})$ whose range is contained in $\range(\bm{W})$. By Lemma~\ref{lemma:constrained_best_low_rank_approximation} we have
\begin{equation*}
    \|g(\bm{A})-\bm{V}\bm{V}^Tg(\bm{A}_{\ell})\|_F^2 \geq \|g(\bm{A}) - (\bm{P}_{\bm{W}} g(\bm{A}))_{\ell}\|_F^2.
\end{equation*}
Hence, we have showed \eqref{eq:low_rank_difference}, which yields the desired inequality. 
\end{proof}
\begin{lemma}\label{lemma:nystrom_truncation}
    Let $\bm{Q} \in \mathbb{R}^{n \times r}$ be an arbitrary orthonormal basis and let
    \begin{equation*}
        \widehat{\bm{A}} = \bm{A} \bm{Q} (\bm{Q}^T \bm{A} \bm{Q})^{\dagger} \bm{Q}^T \bm{A},
    \end{equation*}
    denote the Nyström approximation with respect to $\bm{Q}$. Then, for any Schatten norm $\|\cdot\|_{(s)}$ we have
    \begin{equation*}
        \|\bm{A}-\widehat{\bm{A}}_k\|_{(s)} = \|\bm{A}^{1/2} - (\bm{P}_{\bm{A}^{1/2} \bm{Q}} \bm{A}^{1/2})_k\|_{(2s)}^2.
    \end{equation*}
\end{lemma}
\begin{proof}
Note that
\begin{equation*}
    \widehat{\bm{A}} = \bm{A}^{1/2} \bm{P}_{\bm{A}^{1/2} \bm{Q}}\bm{A}^{1/2} = (\bm{P}_{\bm{A}^{1/2} \bm{Q}}\bm{A}^{1/2})^T (\bm{P}_{\bm{A}^{1/2} \bm{Q}}\bm{A}^{1/2}).
\end{equation*}
Let $\widehat{\bm{P}}^{(k)}$ be the orthogonal projection so that $\widehat{\bm{P}}^{(k)} \bm{A}^{1/2} = \widehat{\bm{P}}^{(k)}\bm{P}_{\bm{A}^{1/2} \bm{Q}}\bm{A}^{1/2} = (\bm{P}_{\bm{A}^{1/2} \bm{Q}}\bm{A}^{1/2})_k$, where we used $\range(\widehat{\bm{P}}_k) \subseteq \range(\bm{P}_{\bm{A}^{1/2} \bm{Q}})$. Hence, we have 
\begin{equation*}
    \widehat{\bm{A}}_k = (\bm{P}_{\bm{A}^{1/2} \bm{Q}}\bm{A}^{1/2})_k^T (\bm{P}_{\bm{A}^{1/2} \bm{Q}}\bm{A}^{1/2})_k = \bm{A}^{1/2} \widehat{\bm{P}}^{(k)}\bm{A}^{1/2}. 
\end{equation*}
Consequently, 
\begin{equation*}
    \|\bm{A}-\widehat{\bm{A}}_k\|_{(s)} = \|\bm{A}^{1/2}(\bm{I}-\widehat{\bm{P}}^{(k)})\bm{A}^{1/2}\|_{(s)} = \|(\bm{I}-\widehat{\bm{P}}^{(k)})\bm{A}^{1/2}\|_{(2s)}^2 = \|\bm{A}^{1/2} - (\bm{P}_{\bm{A}^{1/2} \bm{Q}} \bm{A}^{1/2})_k\|_{(2s)}^2,
\end{equation*}
as required.
\end{proof}
\begin{theorem}
    Let $\bm{Q}$ be an orthonormal basis for 
    \begin{equation*}
        \range\left(\begin{bmatrix} \bm{\Omega} & \bm{A}\bm{\Omega} & \cdots &\bm{A}^q \bm{\Omega} \end{bmatrix} \right),
    \end{equation*}
    where
    \begin{equation*}
        q \geq \frac{\log_2\left(\frac{4n(1+\varepsilon)^2}{\varepsilon}(1+\|\bm{\Omega}_2 \bm{\Omega}_1^{-1}\|_2^2)\right)}{2\sqrt{\varepsilon}}.
    \end{equation*}
    Let 
    \begin{equation*}
        \widehat{\bm{A}} = \bm{A}\bm{Q}(\bm{Q}^T \bm{A} \bm{Q})^{\dagger} \bm{Q}^T \bm{A},
    \end{equation*}
    denote the Nyström approximation of $\bm{A}$. Then, for any operator monotone function $f$ satisfying $f(0) = 0$ we have
    \begin{equation*}
        \|f(\bm{A}) - f(\widehat{\bm{A}}_k)\|_2 \leq (1+2\varepsilon) f(\lambda_{k+1}).
    \end{equation*}
\end{theorem}
\begin{proof}
     Applying Lemma~\ref{lemma:property1} to $g(x) = \sqrt{x}$ gives
    \begin{equation*}
        \|\bm{A}^{1/2} - (\bm{P}_{\bm{A}^{1/2} \bm{Q}} \bm{A}^{1/2})_m\|_{F}^2 \leq \|\bm{A}^{1/2} - \bm{A}_m^{1/2}\|_F^2 + \varepsilon \lambda_{k+1}.
    \end{equation*}
    By \cite[Theorem 3.4]{gu_subspace} we have
    \begin{equation*}
        \|\bm{A}^{1/2} - (\bm{P}_{\bm{A}^{1/2} \bm{Q}} \bm{A}^{1/2})_m\|_{2}^2 \leq \lambda_{m+1} + \varepsilon \lambda_{k+1} \leq (1+2\varepsilon) \lambda_{k+1}.
    \end{equation*}
    Now note that $\bm{A} \succeq \widehat{\bm{A}} \succeq \widehat{\bm{A}}_k \succeq \bm{A}_m \succeq \bm{0}$. Hence, by \cite[Lemma 3.1 (i)]{persson2022randomized} and Lemma~\ref{lemma:nystrom_truncation} we have
    \begin{align*}
        \|\bm{A}-\widehat{\bm{A}}_k\|_2 \leq \|\bm{A}-\widehat{\bm{A}}_m\|_2  = \|\bm{A}^{1/2} - (\bm{P}_{\bm{A}^{1/2} \bm{Q}} \bm{A}^{1/2})_m\|_{2}^2 \leq (1+2\varepsilon) \lambda_{k+1}.
    \end{align*}
    By \cite[Theorem 1]{ando} we have
    \begin{equation*}
        \|f(\bm{A}) - f(\widehat{\bm{A}}_k)\|_2 \leq \|f(\bm{A} - \widehat{\bm{A}}_k)\|_2 = f(\|\bm{A} - \widehat{\bm{A}}_k\|_2) \leq f((1+2\varepsilon)\lambda_{k+1}) \leq (1+2\varepsilon) f(\lambda_{k+1}),
    \end{equation*}
    as required.
\end{proof}


%\textbf{Operator norm}\\
%Suppose that $\|\bm{A} - \widehat{\bm{A}}_k\|_2 \leq (1+\varepsilon) \lambda_{k+1}$. Then,
%\begin{equation*}
 %   \|f(\bm{A})-f(\widehat{\bm{A}}_k)\|_2 \leq \|f(\bm{A}-\widehat{\bm{A}}_k)\|_2 = f(\|\bm{A}-\widehat{\bm{A}}_k\|_2) \leq f((1+\varepsilon) \lambda_{k+1}) \leq (1+\varepsilon) f(\lambda_{k+1}). 
%\end{equation*}
%So how do we get such a guarantee. Let
%\begin{equation*}
 %   \widehat{\bm{A}} = \bm{A}\bm{\Psi}(\bm{\Psi}^T \bm{A} \bm{\Psi})^{-1}\bm{\Psi}^T \bm{A} = \bm{A}^{1/2} \bm{P}_{\bm{A}^{1/2}\bm{\Psi}}\bm{A}^{1/2} = (\bm{P}_{\bm{A}^{1/2}\bm{\Psi}}\bm{A}^{1/2})^T\bm{P}_{\bm{A}^{1/2}\bm{\Psi}}\bm{A}^{1/2},
%\end{equation*}
%where $\bm{\Psi}$ is a sketch (can be from a Krylov subspace). Let $\bm{Q}$ be an orthonormal basis for $\range(\bm{A}^{1/2}\bm{\Psi})$ chosen so that the best rank $k$ approximation of $\bm{Q}\bm{Q}^T \bm{A}^{1/2}$ is $\bm{Q}_{:,1:k}\bm{Q}_{:,1:k}^T \bm{A}^{1/2}$. Hence,
%\begin{equation*}
 %   \widehat{\bm{A}}_k = (\bm{P}_{\bm{A}^{1/2}\bm{\Psi}}\bm{A}^{1/2})_k^T(\bm{P}_{\bm{A}^{1/2}\bm{\Psi}}\bm{A}^{1/2})_k = \bm{A}^{1/2} \bm{Q}_{:,1:k}\bm{Q}_{:,1:k}^T \bm{A}^{1/2}.
%\end{equation*}
%Consequently,
%\begin{equation*}
 %   \|\bm{A}-\widehat{\bm{A}}_k\|_2 = \|(\bm{I}-\bm{Q}_{:,1:k}\bm{Q}_{:,1:k}^T) \bm{A}^{1/2}\|_2^2. 
%\end{equation*}
%The RHS can be bounded using \cite{MM15}. \\\\
\subsection{Per vector guarantees}
\begin{theorem}
    Let $\bm{Q}$ be an orthonormal basis for 
    \begin{equation*}
        \range\left(\begin{bmatrix} \bm{\Omega} & \bm{A}\bm{\Omega} & \cdots &\bm{A}^q \bm{\Omega} \end{bmatrix} \right),
    \end{equation*}
    where
    \begin{equation*}
        q \geq \frac{\log_2\left(\frac{4n(1+\varepsilon)^2}{\varepsilon}(1+\|\bm{\Omega}_2 \bm{\Omega}_1^{-1}\|_2^2)\right)}{2\sqrt{\varepsilon}}.
    \end{equation*}
    Let 
    \begin{equation*}
        \widehat{\bm{A}} = \bm{A}\bm{Q}(\bm{Q}^T \bm{A} \bm{Q})^{\dagger} \bm{Q}^T \bm{A},
    \end{equation*}
    denote the Nyström approximation of $\bm{A}$. Let $\widehat{\lambda}_i$ denote the $i^{\text{th}}$ eigenvalue of $\widehat{\bm{A}}$. Then, for any operator monotone function $f$ satisfying $f(0) = 0$ we have for $i \leq k$
    \begin{equation*}
        0\leq f(\lambda_i) - f(\widehat{\lambda}_i) \leq 3\varepsilon f(\lambda_{k+1}).
    \end{equation*}
\end{theorem}
\begin{proof}
First note that by \cite[Corollary 7.7.4 (c)]{matrixanalysis} we know that the lower bound holds. For the upper bound, note that the eigenvalues of $f(\widehat{\bm{A}})$ and $f(\bm{P}_{\bm{A}^{1/2} \bm{Q}} \bm{A}\bm{P}_{\bm{A}^{1/2}\bm{Q}})$ are the same. Furthermore, by \cite[Theorem V.2.3 (iv), Theorem V.2.5]{bhatia} we know 
\begin{equation*}
    f(\bm{P}_{\bm{A}^{1/2} \bm{Q}} \bm{A}\bm{P}_{\bm{A}^{1/2}\bm{Q}}) \succeq \bm{P}_{\bm{A}^{1/2} \bm{Q}} f(\bm{A})\bm{P}_{\bm{A}^{1/2}\bm{Q}}.
\end{equation*}
Let $s_{i}$ be the $i^{\text{th}}$ eigenvalue of $\bm{P}_{\bm{A}^{1/2} \bm{Q}} f(\bm{A})\bm{P}_{\bm{A}^{1/2}\bm{Q}}$. By \cite[Corollary 7.7.4 (c)]{matrixanalysis} we know $f(\widehat{\lambda}_{i}) \geq s_i$. Hence, it suffices to show that for $i \leq k$ we have
\begin{equation}\label{eq:eigenvalue_inequality}
    0 \leq f(\lambda_i) - s_i \leq 3\varepsilon f(\lambda_{k+1}).
\end{equation}
\David{From this point and onwards we are simply following the proof of \cite[Lemma 9, Property 2]{MM15}. We are basically proving the per vector guarantee for $\bm{P}_{\bm{A}^{1/2} \bm{Q}} f(\bm{A})^{1/2}$. I typed out the proof to make sure everything works out.}
First apply Lemma~\ref{lemma:property1} to the function $g = f^{1/2}$ to obtain
\begin{equation}\label{eq:property2_pt1}
    \|f(\bm{A})^{1/2}-(\bm{P}_{\bm{A}^{1/2}\bm{Q}} f(\bm{A})^{1/2})_{m}\|_F^2 \leq \varepsilon f(\lambda_{k+1}) + \|f(\bm{A})^{1/2} - f(\bm{A}_{m})^{1/2}\|_F^2.
\end{equation}
Let $\widehat{\bm{P}}^{(m)}$ be the projection so that $\widehat{\bm{P}}^{(m)} f(\bm{A})^{1/2} = \widehat{\bm{P}}^{(m)} \bm{P}_{\bm{A}^{1/2}\bm{Q}} f(\bm{A})^{1/2} = (\bm{P}_{\bm{A}^{1/2}\bm{Q}} f(\bm{A})^{1/2})_m$. 
\begin{equation*}
    \|f(\bm{A})^{1/2}-(\bm{P}_{\bm{A}^{1/2}\bm{Q}} f(\bm{A})^{1/2})_{m}\|_F^2 = \|f(\bm{A})^{1/2}-\widehat{\bm{P}}^{(m)}f(\bm{A})^{1/2}\|_F^2 = \tr(f(\bm{A})) - \sum\limits_{i=1}^m s_i.
\end{equation*}
Hence, from \eqref{eq:property2_pt1} we obtain for $i \leq m$
\begin{equation*}
    f(\lambda_i) - s_i \leq \sum\limits_{j=1}^m [f(\lambda_j) - s_j] \leq \varepsilon f(\lambda_{k+1}).
\end{equation*}
Thus, it remains to show \eqref{eq:eigenvalue_inequality} for $i > m$.


Partition $\bm{A}$ as 
\begin{equation*}
    \bm{A} = \begin{bmatrix} \bm{U}_1 & \bm{U}_2^{(1)} & \bm{U}_2^{(2)} \end{bmatrix} \begin{bmatrix} \bm{\Lambda}_1 & & \\ & \bm{\Lambda}_2^{(1)} & \\ & & \bm{\Lambda}_2^{(2)} \end{bmatrix} \begin{bmatrix} \bm{U}_1^T \\ \bm{U}_2^{(1)T} \\ \bm{U}_2^{(2)T}
    \end{bmatrix},
\end{equation*}
where $\bm{\Lambda}_2^{(1)} \in \mathbb{R}^{w \times w}$ contains all singular values $\frac{\lambda_k}{1+\varepsilon} \leq \lambda_i < \lambda_k$. Define
\begin{equation*}
    \bm{A}^{(1)} = \bm{U}_2^{(1)} \bm{\Lambda}_2^{(1)} \bm{U}_2^{(1)T}, \quad \bm{A}^{(2)} = \bm{A} - \bm{A}^{(1)}.
\end{equation*}
Let $\widetilde{p} = \widetilde{p}_{q,\frac{\lambda_k}{1+\varepsilon},\varepsilon,f}$ from Lemma~\ref{lemma:polynomial}. Let $\bm{Y}^{(1)}$ and $\bm{Y}^{(2)}$ be orthonormal bases for $\range(\widetilde{p}(\bm{A}^{(1)}) \bm{\Omega})$ and $\range(\widetilde{p}(\bm{A}^{(2)}) \bm{\Omega})$ respectively. Since $\widetilde{p}(0) = 0$, we know that $\range(\widetilde{p}(\bm{A}^{(1)}))$ and $\range(\widetilde{p}(\bm{A}^{(2)}))$ are orthogonal subspaces. Consequently, $\begin{bmatrix} \bm{Y}^{(1)} & \bm{Y}^{(2)} \end{bmatrix}$ is an orthonormal basis. Furthermore, one can also show that 
\begin{equation*}
    \range(\widetilde{p}(\bm{A}) \bm{\Omega}) \subseteq \range(\begin{bmatrix} \bm{Y}^{(1)} & \bm{Y}^{(2)} \end{bmatrix})
\end{equation*}
\David{It would be good to show the statement above formally, and attach it here.} Hence, for any $\bm{x} \in \range(\widetilde{p}(\bm{A}) \bm{\Omega})$ there exists $\bm{x}^{(1)} \in \range(\bm{Y}^{(1)})$ and $\bm{x}^{(2)} \in \range(\bm{Y}^{(2)})$ such that $\bm{x} = \bm{x}^{(1)} + \bm{x}^{(2)}$. Hence, for any $\bm{x}\in \range(\widetilde{p}(\bm{A})$ we have
\begin{equation}\label{eq:decomposition}
    \|g(\bm{A})\bm{x}\|_F^2 =  \|g(\bm{A})\bm{x}^{(1)}\|_F^2 +  \|g(\bm{A})\bm{x}^{(2)}\|_F^2.
\end{equation}
Moreover, since $g = f^{1/2}$ \David{we crucially use concavity here}
\begin{equation}\label{eq:first_inequality}
    \|g(\bm{A})\bm{x}^{(1)}\|_2^2 \geq f\left(\frac{\lambda_k}{1+\varepsilon}\right)\|\bm{x}^{(1)}\|_2^2 \geq \frac{1}{1+\varepsilon} f(\lambda_k) \|\bm{x}^{(1)}\|_2^2.
\end{equation}
Furthermore,
\begin{align*}
    &\|\widetilde{p}(\bm{A}^{(2)})-\bm{Y}^{(2)}\bm{Y}^{(2)T}\widetilde{p}(\bm{A}^{(2)})\|_F^2 \leq (1+\|\bm{\Omega}_2\bm{\Omega}_1^{-1}\|_2^2)\sum\limits_{i=k+w+1}^n \widetilde{p}(\lambda_i)^2 \leq \\
    &\frac{4n}{2^{2\sqrt{\varepsilon}q}}(1+\|\bm{\Omega}_2\bm{\Omega}_1^{-1}\|_2^2) f(\lambda_k) \leq \varepsilon f(\lambda_k).
\end{align*}
Furthermore, using the same technique as in Lemma~\ref{lemma:property1} and using $\bm{A}_k = \bm{A}^{(1)}_k$ we can show 
\begin{equation*}
    \|g(\bm{A}_{k}) - \bm{Y}^{(2)}\bm{Y}^{(2)T}g(\bm{A}_{k})\|_F^2 \leq \|\widetilde{p}(\bm{A}^{(2)})-\bm{Y}^{(2)}\bm{Y}^{(2)T}\widetilde{p}(\bm{A}^{(2)})\|_F^2 \leq \varepsilon f(\lambda_k).
\end{equation*}
Hence, following \cite[Equation (11)]{MM15} we have for any $\bm{x}^{(2)} \in \range(\bm{Y}^{(2)})$ that
\begin{equation}\label{eq:second_inequality}
    (1-\varepsilon)f(\lambda_k)\|\bm{x}^{2}\|_2^2 \leq \|g(\bm{A})\bm{x}^{(2)}\|_2^2.
\end{equation}
Combining \eqref{eq:first_inequality} and \eqref{eq:second_inequality} with \eqref{eq:decomposition} we get for any $\bm{x} \in \range(\widetilde{p}(\bm{A}\bm{\Omega}))$ with unit norm we have
\begin{equation*}
    \|g(\bm{A})\bm{x}\|_2^2 \geq (\frac{1}{1+\varepsilon}\|\bm{x}^{(1)}\|_2^2 + (1-\varepsilon)\|\bm{x}^{(2)}\|_2^2)f(\lambda_k) \geq (1-2\varepsilon)f(\lambda_k).
\end{equation*}
Now let $\widetilde{\bm{u}}_{\ell}$ be the $\ell^{\text{th}}$ eigenvector of $\bm{P}_{\widetilde{p}(\bm{A})\bm{\Omega}} f(\bm{A})\bm{P}_{\widetilde{p}(\bm{A})\bm{\Omega}}$ and let $\widetilde{s}_{\ell}$ denote the $\ell^{\text{th}}$ eigenvalue.
Hence, 
\begin{equation*}
    \widetilde{s}_{\ell} = \widetilde{\bm{u}}_{\ell}^T\bm{P}_{\widetilde{p}(\bm{A})\bm{\Omega}} f(\bm{A})\bm{P}_{\widetilde{p}(\bm{A})\bm{\Omega}}\widetilde{\bm{u}}_{\ell} = \widetilde{\bm{u}}_{\ell}^Tf(\bm{A})\widetilde{\bm{u}}_{\ell} = \|g(\bm{A})\widetilde{\bm{u}}_{\ell}\|_2^2 \leq (1-2\varepsilon)f(\lambda_k)
\end{equation*}
Since $\range(\widetilde{p}(\bm{A})\bm{\Omega}) \subseteq \range(\bm{A}^{1/2} \bm{Q})$ we know that $s_{\ell} \geq \widetilde{s}_{\ell}$. Consequently, for $\ell > m$ we have \David{we crucially use concavity here}
\begin{align*}
    &0 \leq f(\lambda_{\ell}) - s_{\ell} \leq f(\lambda_{\ell}) - \widetilde{s}_{\ell} \leq f((1+\varepsilon) \lambda_{k+1}) - (1-2\varepsilon)f(\lambda_k) \leq \\
    &(1+\varepsilon) f(\lambda_{k+1}) - (1-2\varepsilon) f(\lambda_k) \leq (1+\varepsilon) f(\lambda_{k+1}) - (1-2\varepsilon) f(\lambda_{k+1}) \leq 3\varepsilon f(\lambda_{k+1}),
\end{align*}
as required.
\end{proof}
%\textbf{Per vector}\\
%Note that for per-vector guarantees we have that the eigenvalues of $f(\widehat{\bm{A}})$ are the same as the ones of $f(\bm{P}_{\bm{A}^{1/2} \bm{\Psi}} \bm{A}\bm{P}_{\bm{A}^{1/2} \bm{\Psi}})$. But we also know 
%\begin{equation*}
    %f(\bm{P}_{\bm{A}^{1/2} \bm{\Psi}} \bm{A}\bm{P}_{\bm{A}^{1/2} \bm{\Psi}}) \succeq \bm{P}_{\bm{A}^{1/2} \bm{\Psi}} f(\bm{A})\bm{P}_{\bm{A}^{1/2} \bm{\Psi}} = (\bm{P}_{\bm{A}^{1/2} \bm{\Psi}} f(\bm{A})^{1/2})(\bm{P}_{\bm{A}^{1/2} \bm{\Psi}} f(\bm{A})^{1/2})^T.
%\end{equation*}
%Hence, we can obtain per vector guarantees as well.\\\\
\subsection{Nuclear norm guarantees}
\begin{theorem}
    Let $\bm{Q}$ be an orthonormal basis for 
    \begin{equation*}
        \range\left(\begin{bmatrix} \bm{\Omega} & \bm{A}\bm{\Omega} & \cdots &\bm{A}^q \bm{\Omega} \end{bmatrix} \right),
    \end{equation*}
    where
    \begin{equation*}
        q \geq \frac{\log_2\left(\frac{4n(1+\varepsilon)^2}{\varepsilon}(1+\|\bm{\Omega}_2 \bm{\Omega}_1^{-1}\|_2^2)\right)}{2\sqrt{\varepsilon}}.
    \end{equation*}
    Let 
    \begin{equation*}
        \widehat{\bm{A}} = \bm{A}\bm{Q}(\bm{Q}^T \bm{A} \bm{Q})^{\dagger} \bm{Q}^T \bm{A},
    \end{equation*}
    denote the Nyström approximation of $\bm{A}$. Then, for any operator monotone function $f$ satisfying $f(0) = 0$ we have
    \begin{equation*}
        \|f(\bm{A}) - f(\widehat{\bm{A}}_k)\|_* \leq (1+\varepsilon) \|f(\bm{A})-f(\bm{A}_k)\|_*.
    \end{equation*}
\end{theorem}
\begin{proof}
Let $\bm{W}$ and $\widetilde{\bm{W}}$ be an orthonormal bases for $\bm{A}^{1/2}\bm{Q}$ chosen so that 
\begin{equation*}
    \bm{W}_{:,1:\ell}\bm{W}_{:,1:\ell}^T \bm{A}^{1/2} = (\bm{W}\bm{W}^T \bm{A}^{1/2})_{\ell}, \quad \widetilde{\bm{W}}_{:,1:\ell}\widetilde{\bm{W}}_{:,1:\ell}^T f(\bm{A})^{1/2} = (\widetilde{\bm{W}}\widetilde{\bm{W}}^T f(\bm{A})^{1/2})_{\ell}.
\end{equation*}
Note that we have for $i \leq \ell$
\begin{align}\label{eq:singular_value_inequality}
    \begin{split}
    &\sigma_i(\widetilde{\bm{W}}_{:,1:\ell}\widetilde{\bm{W}}_{:,1:\ell}^T \bm{A}^{1/2}) = \sigma_i(\widetilde{\bm{W}}_{:,1:\ell}\widetilde{\bm{W}}_{:,1:\ell}^T \bm{W}\bm{W}^T\bm{A}^{1/2}) \leq \\
    &\sigma_1(\widetilde{\bm{W}}_{:,1:\ell}\widetilde{\bm{W}}_{:,1:\ell}^T )\sigma_i(\bm{W}\bm{W}^T\bm{A}^{1/2}) = \sigma_i(\bm{W}_{:,1:\ell}\bm{W}_{:,1:\ell}^T\bm{A}^{1/2}).
    \end{split}
\end{align}
Furthermore, we have
\begin{equation}\label{eq:nystrom_lowrank}
    \widehat{\bm{A}}_k = (\bm{W}_{:,1:\ell}\bm{W}_{:,1:k}^T \bm{A}^{1/2})^T(\bm{W}_{:,1:k}\bm{W}_{:,1:k}^T \bm{A}^{1/2}).
\end{equation}
Hence, using $f(\bm{A}) \succeq f(\widehat{\bm{A}}_k)$, \eqref{eq:singular_value_inequality}, and \eqref{eq:nystrom_lowrank} we have
\begin{align*}
    &\|f(\bm{A}) - f(\widehat{\bm{A}}_k)\|_* = \tr(f(\bm{A})) - \tr(f(\widehat{\bm{A}}_k)) = \tr(f(\bm{A})) - \sum\limits_{i=1}^k f(\sigma_i(\bm{W}_{:,1:k}\bm{W}_{:,1:k}^T\bm{A}^{1/2})^2) \leq \\
    &\tr(f(\bm{A})) - \sum\limits_{i=1}^k f(\sigma_i(\widetilde{\bm{W}}_{:,1:k}\widetilde{\bm{W}}_{:,1:k}^T\bm{A}^{1/2})^2) = \tr(f(\bm{A})) - \tr(f(\widetilde{\bm{W}}_{:,1:k}\widetilde{\bm{W}}_{:,1:k}^T\bm{A}\widetilde{\bm{W}}_{:,1:k}\widetilde{\bm{W}}_{:,1:k}^T)).
\end{align*}
Using \cite[Theorem V.2.3 (iv), Theorem V.2.5]{bhatia} we have
\begin{align*}
    &\tr(f(\bm{A})) - \tr(f(\widetilde{\bm{W}}_{:,1:k}\widetilde{\bm{W}}_{:,1:k}^T\bm{A}\widetilde{\bm{W}}_{:,1:k}\widetilde{\bm{W}}_{:,1:k}^T){} \leq \tr(f(\bm{A})) - \tr(\widetilde{\bm{W}}_{:,1:k}\widetilde{\bm{W}}_{:,1:k}^Tf(\bm{A})\widetilde{\bm{W}}_{:,1:k}\widetilde{\bm{W}}_{:,1:k}^T) = \\
    &\|f(\bm{A})^{1/2} - \widetilde{\bm{W}}_{:,1:k}\widetilde{\bm{W}}_{:,1:k}^Tf(\bm{A})^{1/2}\|_F^2.
\end{align*}
Hence,
\begin{equation*}
    \|f(\bm{A}) - f(\widehat{\bm{A}}_k)\|_* \leq \|f(\bm{A})^{1/2} - \widetilde{\bm{W}}_{:,1:k}\widetilde{\bm{W}}_{:,1:k}^Tf(\bm{A})^{1/2}\|_F^2.
\end{equation*}
\David{The rest of the proof would follow the proof of Property 3.}

\end{proof}

\begin{theorem}
    FROBENIUS NORM RESULT.
\end{theorem}
\begin{proof}
Proof outline:
\begin{itemize}
    \item Reduce to the case when $\bm{A}$ is diagonal and has full rank.
    \item When $\bm{A}$ has full rank, it is invertible. Then $\bm{A}^{1/2} \bm{Q} = f(\bm{A})^{1/2} (f(\bm{A})^{-1/2} \bm{A}^{1/2} \bm{Q}) = f(\bm{A})^{1/2} \bm{\Psi}$, and $\bm{\Psi}$ is a random matrix that points "more" in the correct directions than $\bm{Q}$. This is because $\sqrt{x/f(x)}$ is an increasing function. 
    \item Now use arguments that shows that subspace iteration monotonically decreases the error. 
\end{itemize}
\end{proof}
%Note that
%\begin{equation*}
    %\|f(\bm{A})-f(\widehat{\bm{A}_r})\|_* \leq \|(\bm{I}-\bm{Q}_{:,1:k}\bm{Q}_{:,1:k}^T) f(\bm{A})^{1/2}\|_F^2. 
%\end{equation*}
%So we can get nuclear norm guarantees as well.


\textbf{TODOS}
\begin{itemize}
    \item Adding properties of concave functions
    \begin{enumerate}
        \item $f(tx) \leq tf(x)$ for $t \geq 1$ and $f(tx) \leq tf(x)$ for $t \leq 1$;
        \item $f(x)/x$ is decreasing.
    \end{enumerate}
\end{itemize}

\section{Running Block Lanczos on the inverse function}
\begin{lemma}\label{lemma:krylov_inverse}
Let $g$ be any convex and increasing function satisfying $g(0) = 0$.\footnote{Operator monotone functions are very smooth, $C^{\infty}$ on $(0,\infty)$ even, but I am not sure if operator monotone implies strictly increasing. We would need strictly increasing to define an inverse.} Let $\gamma \in (0,1]$ and $\alpha > 0$. Then,
the function
\begin{equation*}
    p(x) = \frac{(1+\gamma)\alpha T_q\left(\frac{g(x)}{g(\alpha)}\right)}{T_q\left(\frac{g((1+\gamma)\alpha)}{g(\alpha)}\right)}
\end{equation*}
satisfies
\begin{enumerate}
    \item[(i)] $p(x) \geq x$ for $x \geq (1+\gamma) \alpha$;
    \item[(ii)] $p(x) \leq \frac{2(1+\gamma)\alpha}{2^{q\sqrt{\gamma}}}$ for $x \in [0,\alpha]$.
\end{enumerate}
Furthermore, the function
\begin{equation*}
    \widetilde{p}(x) = \sqrt{\frac{g(x)}{g((1+\gamma)\alpha)}}p(x),
\end{equation*}
satisfies the same bound. \David{The second function would deal with the half iteration of that we see for the Nyström approximation.}
\end{lemma}
\begin{proof}
\David{The result would almost follow immediately from Lemma~\ref{lemma:polynomial}, so I should not have reproven it... Furthermore, check if operator monotone functions are strictly increasing and if we would have any issues with $x$ falling outside the domain of $g$. For the strictly increasing part, I think this might follow from the integral representation of operator monotone functions. Clearly we are assuming that $f(x) = 0$ not everywhere. }Note that $p((1+\gamma)\alpha) = (1+\gamma)\alpha$. Hence to show $(i)$ we only need to show that $p'(x) \geq 1$ for $x \geq (1+\gamma)\alpha$. Since $p$ is a composition of to convex functions on $x \geq (1+\gamma)\alpha$ we only need to show that $p'((1+\gamma)\alpha) \geq 1$. Note that
\begin{equation*}
    p'((1+\gamma)\alpha) = \frac{(1+\gamma)\alpha \frac{g'((1+\gamma)\alpha)}{g(\alpha)}T'_q(\frac{g((1+\gamma)\alpha)}{g(\alpha)})}{T_q\left(\frac{g((1+\gamma)\alpha)}{g(\alpha)}\right)} = \frac{(1+\gamma)\alpha g'((1+\gamma)\alpha)}{g((1+\gamma)\alpha)} \cdot \frac{\frac{g((1+\gamma)\alpha)}{g(\alpha)}T_q'\left(\frac{g((1+\gamma)\alpha)}{g(\alpha)}\right)}{T_q\left(\frac{g((1+\gamma)\alpha)}{g(\alpha)}\right)}.
\end{equation*}
Note that $\frac{g((1+\gamma)\alpha)}{g(\alpha)} \geq 1$ so for some $\eta \geq 0$ we can write $\frac{g((1+\gamma)\alpha)}{g(\alpha)} = 1+\eta$. Furthermore, let $y = (1+\gamma)\alpha$. Hence, it suffices to show
\begin{equation*}
    \frac{y g'(y)}{g(y)} \geq 1, \quad \frac{(1+\eta) T_q'(1+\eta)}{T_q(1+\eta)} \geq 1.
\end{equation*}
The second statement was shown in \cite[Lemma 5]{MM15}. The first statement is a consequence of convexity: Note that for any $z$ we have $g(z) \geq g(y) + g'(y)(z-y)$. Set $z = 0$ and use $g(0) = 0$. This yields $(i)$.

We now proceed with proving $(ii)$. Since $g$ is increasing and $|T_q(z)|\leq 1$ for $z \in [0,1]$ we only need to show
\begin{equation*}
    T_q\left(\frac{g((1+\gamma)\alpha)}{g(\alpha)}\right) \geq 2^{q\sqrt{\gamma}-1}
\end{equation*}
By convexity of $g$ we have
\begin{equation*}
    \frac{g((1+\gamma)\alpha)}{g(\alpha)} \geq \frac{(1+\gamma)g(\alpha)}{g(\alpha)} = (1+\gamma).
\end{equation*}
Hence, since $T_q(x)$ is increasing for $x \geq 1$ we have
\begin{equation*}
    T_q\left(\frac{g((1+\gamma)\alpha)}{g(\alpha)}\right)\geq T_q(1+\gamma).
\end{equation*}
From \cite[Lemma 5]{MM15} we know that $T_q(1+\gamma) \geq 2^{q\sqrt{\gamma}-1}$, which yields $(ii)$. 

The claim for the function $\widetilde{p}$ follows from the fact that $\sqrt{\frac{g(x)}{g((1+\gamma)\alpha)}} \leq 1$ whenever $x \leq (1+\gamma)\alpha$ and $\sqrt{\frac{g(x)}{g((1+\gamma)\alpha)}} \geq 1$ whenever $x\geq (1+\gamma)\alpha$.
\end{proof}

\section{Optimality in the Schatten 4-norm}
We want to show that
\begin{equation*}
    \|(\bm{I}-\bm{Q}\bm{Q}^T)\bm{A}\|_{(4)}^2 \leq (1+\varepsilon)\|\bm{A}-\bm{A}_k\|_{(4)}^2.
\end{equation*}
We know that by running $q = O(\frac{\log(n/\varepsilon)}{\sqrt{\varepsilon}})$ iterations of Lanczos on $\bm{A}\bm{A}^T$ we have
\begin{equation*}
    \|(\bm{I}-\bm{Q}\bm{Q}^T)\bm{A}\bm{A}^T\|_F^2 \leq (1+\varepsilon)\|\bm{A}\bm{A}^T-\bm{A}_k\bm{A}_k^T\|_F^2 = (1+\varepsilon)\|\bm{A}-\bm{A}_k\|_{(4)}^4.
\end{equation*}
Hence,
\begin{align*}
    &\|(\bm{I}-\bm{Q}\bm{Q}^T)\bm{A}\|_{(4)}^2 = \|(\bm{I}-\bm{Q}\bm{Q}^T)\bm{A}\bm{A}^T(\bm{I}-\bm{Q}\bm{Q}^T)\|_{F} \leq \|(\bm{I}-\bm{Q}\bm{Q}^T)\bm{A}\bm{A}^T\|_F \leq \\
    &\sqrt{1+\varepsilon}\|\bm{A}-\bm{A}_k\|_{(4)}^2 \leq (1+\varepsilon)\|\bm{A}-\bm{A}_k\|_{(4)}^2.
\end{align*}

\section{Near optimality of two sided projections}
\begin{theorem}\label{theorem:two_sided_frobenius}
    Let $\bm{A}$ be an SPSD matrix and assume that $\bm{Q}$ be any basis so that 
    \begin{equation*}
        \|(\bm{I}-\bm{P}_{\bm{Q}})\bm{A}\|_F^2 \leq (1+\varepsilon)\|\bm{A} - \bm{A}_k\|_F^2.
    \end{equation*}
    Then,
    \begin{equation*}
        \|\bm{A} - \bm{P}_{\bm{A}\bm{Q}}\bm{A}\bm{P}_{\bm{A}\bm{Q}}\|_F^2 \leq \|(\bm{I}-\bm{P}_{\bm{Q}})\bm{A}\|_F^2 \leq (1+\varepsilon)\|\bm{A} - \bm{A}_k\|_F^2.
    \end{equation*}
\end{theorem}
\begin{proof}
First note that the best low-rank approximation whose range falls in $\range(\bm{A} \bm{Q})$ is $\bm{P}_{\bm{A} \bm{Q}} \bm{A}$. Similarly, the best low-rank approximation whose range and co-range falls in $\range(\bm{A}\bm{Q})$ is $\bm{P}_{\bm{A}\bm{Q}}\bm{A}\bm{P}_{\bm{A}\bm{Q}}$. Consequently, since the Nyström approximation is a low-rank approximation whose range and co-range falls in $\range(\bm{A}\bm{Q})$ we have
\begin{equation}\label{eq:range}
    \|\bm{A} - \bm{P}_{\bm{A}\bm{Q}}\bm{A}\|_F^2 \leq \|\bm{A} - \bm{P}_{\bm{A}\bm{Q}}\bm{A}\bm{P}_{\bm{A}\bm{Q}}\|_F^2 \leq \|\bm{A} - \bm{A}\bm{Q}(\bm{Q}^T \bm{A}\bm{Q})^{-1}\bm{Q}^T \bm{A}\|_F^2.
\end{equation}
Furthermore, we have
\begin{align}\label{eq:nystrom_to_onesided}
\begin{split}
     &\|\bm{A} - \bm{A}\bm{Q}(\bm{Q}^T \bm{A}\bm{Q})^{-1}\bm{Q}^T \bm{A}\|_F^2 = \|\bm{A}^{1/2}(\bm{I} - \bm{P}_{\bm{A}^{1/2} \bm{Q}})\bm{A}^{1/2} \|_F^2 = \\
     &\|(\bm{I} - \bm{P}_{\bm{A}^{1/2} \bm{Q}})\bm{A}(\bm{I} - \bm{P}_{\bm{A}^{1/2} \bm{Q}})\|_F^2 \leq \|(\bm{I} - \bm{P}_{\bm{A}^{1/2} \bm{Q}})\bm{A}\|_F^2.
     \end{split}
\end{align}
Combining \eqref{eq:range} and \eqref{eq:nystrom_to_onesided} yields
\begin{equation*}
     \|\bm{A} - \bm{P}_{\bm{A}\bm{Q}}\bm{A}\|_F^2 \leq \|\bm{A} - \bm{P}_{\bm{A}\bm{Q}}\bm{A}\bm{P}_{\bm{A}\bm{Q}}\|_F^2 \leq \|(\bm{I} - \bm{P}_{\bm{A}^{1/2} \bm{Q}})\bm{A}\|_F^2.
\end{equation*}
Continuing the same argument on $\|(\bm{I} - \bm{P}_{\bm{A}^{1/2} \bm{Q}})\bm{A}\|_F^2$ gives
\begin{equation*}
    \|\bm{A} - \bm{P}_{\bm{A}\bm{Q}}\bm{A}\bm{P}_{\bm{A}\bm{Q}}\|_F^2 \leq \|(\bm{I}-\bm{P}_{\bm{Q}})\bm{A}\|_F^2 \leq (1+\varepsilon) \|\bm{A}-\bm{A}_k\|_F^2,
\end{equation*}
as required. 
\end{proof}

%\begin{theorem}
 %   Let $\bm{A}$ be an SPSD matrix and assume that $\bm{Q} \in \mathbb{R}^{n \times k}$ be any basis so that 
  %  \begin{equation*}
   %     \|(\bm{I}-\bm{P}_{\bm{Q}})\bm{A}\|_F^2 \leq \|\bm{A} - \bm{A}_{m}\|_F^2 + \varepsilon \sigma_{k+1}^2,
    %\end{equation*}
    %where $m$ is chosen so that $\sigma_m > (1+\varepsilon)\sigma_{k+1}$ and $\sigma_{m+1} \leq  (1+\varepsilon)\sigma_{k+1}$. 
    %Then,
    %\begin{equation*}
     %   \|\bm{A} - \bm{P}_{\bm{A}\bm{Q}}\bm{A}\bm{P}_{\bm{A}\bm{Q}}\|_2^2 \leq (1+\varepsilon)\|\bm{A} - \bm{A}_k\|_2^2.
    %\end{equation*}
%\end{theorem}
%\begin{proof}
%By the argument in Theorem~\ref{theorem:two_sided_frobenius} we know that
%\begin{equation*}
 %   \|\bm{A} - \bm{P}_{\bm{A}\bm{Q}}\bm{A}\bm{P}_{\bm{A}\bm{Q}}\|_F^2 \leq \|\bm{A} - \bm{A}_{m}\|_F^2 + \varepsilon \sigma_{k+1}^2
%\end{equation*}
%\end{proof}


\section{Checking the 3 properties}
Consider $\bm{A} \in \mathbb{R}^{m \times n}$, where $m \geq n$, with SVD
\begin{equation*}
    \bm{A} = \bm{U} \bm{\Sigma} \bm{V}^T = \begin{bmatrix} \bm{U}_1 & \bm{U}_2 \end{bmatrix} \begin{bmatrix} \bm{\Sigma}_1 & \\ & \bm{\Sigma}_2 \end{bmatrix} \begin{bmatrix} \bm{V}_1^T \\ \bm{V}_2^T \end{bmatrix},
\end{equation*}
where $\bm{\Sigma}_1 \in \mathbb{R}^{k \times k}$ contains the $k$ largest singular values on the diagonal and $\bm{U}_1 \in \mathbb{R}^{m \times k}$ and $\bm{V}_1 \in \mathbb{R}^{n \times k}$ are the corresponding singular vectors. Let $\bm{\Omega} \in \mathbb{R}^{n \times k}$ be a sketching matrix so that $\bm{\Omega}_1 = \bm{V}_1^T \bm{\Omega}$ has full rank. Furthermore, define $\bm{\Omega}_2 = \bm{V}_2^T \bm{\Omega}$. Let $g:[0,\infty) \mapsto [0,\infty)$ be an increasing function and let $p_1 = p_1^{(q,\gamma)}, p_1 = p_2^{(q,\gamma)}: [0,\infty) \mapsto [0,\infty)$ be functions, paramatrized by $q \in \mathbb{N}$ and $\gamma \in (0,1]$, so that
\begin{align*}
    &p_1(x) \geq g(x) \text{ for } x \geq (1+\gamma) \sigma_{k+1}, \quad &&p_2(x) \geq g(x) \text{ for } x \geq \sigma_{k}, \\
    &|p_1(x)|^2 \leq \varepsilon^{(q,\gamma)} \sigma_{k+1}^2 \text{ for } x \in [0,\sigma_{k+1}], \quad &&|p_2(x)|^2 \leq \frac{\varepsilon^{(q,\gamma)} \sigma_k^2}{(1+\gamma)^2} \text{ for } x \in \left[0, \frac{\sigma_k}{1+\gamma} \right]. 
\end{align*}
Let $\bm{Y}_1 \in \mathbb{R}^{n \times k}$ and $\bm{Y}_2 \in \mathbb{R}^{n \times k}$ be orthonormal bases for $\range(\bm{U} p_1(\bm{\Sigma}) \bm{V}^T \bm{\Omega})$ and $\range(\bm{U} p_2(\bm{\Sigma}) \bm{V}^T \bm{\Omega})$ respectively, and $\bm{Q}$ is an orthonormal basis whose range contains the ranges of $\bm{Y}_1$ and $\bm{Y}_2$. Without loss of generality we may choose $\bm{Q}$ so that $\bm{Q}_{:,1:\ell}\bm{Q}_{:,1:\ell}^T g(\bm{A}) = (\bm{Q}\bm{Q}^T g(\bm{A}))_{\ell}$. 
\begin{theorem}
    Let $m$ be the number of singular values so that $(1+\gamma) g(\sigma_{k+1})$, and let $w$ be the number of singular values so that $\frac{1}{1+\gamma}g(\sigma_k) \leq g(\sigma_i) < g(\sigma_k)$. Define
    \begin{equation*}
        \delta= n(1+\|\bm{\Omega}_2\bm{\Omega}_1^{-1}\|_2^2) \varepsilon^{(q,\gamma)}
    \end{equation*}
    and assume $\delta < 1.$ Then,
    \begin{itemize}
        \item[1.] For all $\ell \leq m$ we have $\|g(\bm{A}) - \bm{Q}_{:,1:\ell}\bm{Q}_{:,1:\ell}^T g(\bm{A})\|_F^2 \leq \|g(\bm{A}) - g(\bm{A})_{\ell}\|_F^2 + \delta g(\sigma_{k+1})^2$,
    \end{itemize}
    and for $\gamma = \delta$ we have
    \begin{itemize}
        \item[2.] for all $\ell \leq k$ we have $g(\sigma_{\ell})^2 - \sigma_{\ell}(\bm{Q}\bm{Q}^T g(\bm{A}))^2 \leq 4\delta g(\sigma_{k+1})^2$;
        \item[3.] for all $\ell \leq k$ we have $\|g(\bm{A}) - \bm{Q}_{:,1:\ell}\bm{Q}_{:,1:\ell}^T g(\bm{A})\|_F^2 \leq \|g(\bm{A}) - g(\bm{A})_{\ell}\|_F^2 + 6(w+1)\delta \sigma_{k+1}^2$.
    \end{itemize}
\end{theorem}
\David{We should probably only prove 2 and 3 whenever $\gamma = \delta$.}

\section{Black boxing eigenvalue guarantees}
Suppose that the eigenvalues of $\widehat{\bm{A}}$ satisfies
\begin{equation}\label{eq:eigvals}
    0 \leq \lambda_{i} - \widehat{\lambda}_{i} \leq \varepsilon \lambda_{k+1}, \quad i = 1,\cdots,k,
\end{equation}
where $\varepsilon \in [0,1]$. (Note that we can do the same proof with only the assumption $|\lambda_i - \widehat{\lambda_i}| \leq \varepsilon \lambda_{k+1}$ because if $\lambda_i \leq \widehat{\lambda}_i$ then we can just interchange $\lambda_i$ and $\widehat{\lambda}_{i}$ them in the proof)
Note that for any $t \in [0,1]$ we have $f(tx) \geq tf(x)$ for a concave function $f$ with $f(0)=0$. Consequently,
\begin{equation}\label{eq:diff}
    \frac{f(\lambda_{k+1}) - f((1-\varepsilon)\lambda_{k+1})}{\varepsilon} \leq \frac{f(\lambda_{k+1}) - (1-\varepsilon)f(\lambda_{k+1})}{\varepsilon} = f(\lambda_{k+1}).
\end{equation}
Now note that the function
\begin{equation*}
    g(t) = \frac{f(t) - f(t-\varepsilon \lambda_{k+1})}{\varepsilon}
\end{equation*}
is decreasing because
\begin{equation*}
    g'(t) = \frac{f'(t) - f'(t-\varepsilon \lambda_{k+1})}{\varepsilon} \leq 0
\end{equation*}
because $f'' \leq 0$ ($f'$ is a decreasing function and $t \geq t - \varepsilon \lambda_{k+1}$). Consequently, for any $i = 1,\ldots,k$
\begin{equation}\label{eq:diff2}
    \frac{f(\lambda_{k+1}) - f((1-\varepsilon)\lambda_{k+1})}{\varepsilon} \geq \frac{f(\lambda_i) - f(\lambda_i-\varepsilon \lambda_{k+1})}{\varepsilon}.
\end{equation}
Hence, by \eqref{eq:diff} and \eqref{eq:diff2} we know
\begin{equation*}
    f(\lambda_{k+1}) \geq \frac{f(\lambda_i) - f(\lambda_i-\varepsilon \lambda_{k+1})}{\varepsilon},
\end{equation*}
which implies 
\begin{equation*}
    f(\lambda_i - \varepsilon \lambda_{k+1}) \geq f(\lambda_i)-\varepsilon f(\lambda_{k+1}).
\end{equation*}
Moreover, from \eqref{eq:eigvals} we know
\begin{equation*}
    f(\widehat{\lambda}_i) \geq f(\lambda_i - \varepsilon \lambda_{k+1}) \geq f(\lambda_i)-\varepsilon f(\lambda_{k+1}).
\end{equation*}
Hence, we can black box the eigenvalue guarantees. 

\section{Black boxing nuclear norm}
Suppose that $\|\bm{A}-\widehat{\bm{A}}_k\|_* \leq (1+\varepsilon)\|\bm{A}-\bm{A}_k\|_*$. This implies that
\begin{equation}\label{eq:tracediff}
    \sum\limits_{i=1}^k (\lambda_i - \widehat{\lambda}_i) \leq \varepsilon \sum\limits_{i=k+1}^n \lambda_i.
\end{equation}
Let us define $(1-\delta_i) = \frac{\widehat{\lambda}_i}{\lambda_i}$. Hence, \eqref{eq:tracediff} implies that
\begin{equation}
    \sum\limits_{i=1}^k \delta_i \lambda_i \leq \varepsilon \sum\limits_{i=k+1}^n \lambda_i.
\end{equation}
We want to show that
\begin{equation*}
    \sum\limits_{i=1}^k (f(\lambda_i) - f(\widehat{\lambda}_i)) \leq \varepsilon \sum\limits_{i=k+1}^n f(\lambda_i).
\end{equation*}
Note that since $f(tx) \geq tf(x)$ for $t \in [0,1]$ we have
\begin{equation*}
    \sum\limits_{i=1}^k (f(\lambda_i) - f(\widehat{\lambda}_i)) \leq \sum\limits_{i=1}^k \delta_if(\lambda_i).
\end{equation*}
Hence, we just need to show that 
\begin{equation*}
    \sum\limits_{i=1}^k \delta_if(\lambda_i) \leq \varepsilon \sum\limits_{i=k+1}^n f(\lambda_i).
\end{equation*}
We will show
\begin{equation*}
    \frac{1}{\varepsilon} \leq \frac{\sum\limits_{i=k+1}^n \lambda_i}{\sum\limits_{i=1}^k \delta_i\lambda_i} \leq \frac{\sum\limits_{i=k+1}^n f(\lambda_i)}{\sum\limits_{i=1}^k \delta_i f(\lambda_i)}
\end{equation*}
Note that for $i = 1,\cdots,k$
\begin{align*}
    &\frac{\lambda_{k+j}}{\lambda_i} \leq \frac{f(\lambda_{k+j})}{f(\lambda_i)}\\
    \Rightarrow &\frac{\lambda_{k+j}}{\delta_i\lambda_i} \leq \frac{f(\lambda_{k+j})}{\delta_if(\lambda_i)}\\
    \Rightarrow &\frac{\sum\limits_{j=k+1}^n\lambda_{j}}{\delta_i\lambda_i} \leq \frac{\sum\limits_{j=k+1}^nf(\lambda_{j})}{\delta_if(\lambda_i)}\\
    \Rightarrow &\frac{\delta_i\lambda_i}{\sum\limits_{j=k+1}^n\lambda_{j}} \geq \frac{\delta_if(\lambda_i)}{\sum\limits_{j=k+1}^nf(\lambda_{j})}\\
    \Rightarrow &\frac{\sum\limits_{i=1}^k\delta_i\lambda_i}{\sum\limits_{j=k+1}^n\lambda_{j}} \geq \frac{\sum\limits_{i=1}^k\delta_if(\lambda_i)}{\sum\limits_{j=k+1}^nf(\lambda_{j})}\\
    \Rightarrow &\frac{\sum\limits_{j=k+1}^n\lambda_{j}}{\sum\limits_{i=1}^k\delta_i\lambda_i} \leq \frac{\sum\limits_{j=k+1}^nf(\lambda_{j})}{\sum\limits_{i=1}^k\delta_if(\lambda_i)},
\end{align*}
as required. 

\section{Black boxing Frobenius norm}
An entirely identical argument as the Nuclear norm (but square all eigenvalues) will show that if 
\begin{equation*}
    \|\bm{A}\|_F^2 - \|\widehat{\bm{A}}_k\|_F^2 \leq (1+\varepsilon)\|\bm{A}-\bm{A}_k\|_F^2
\end{equation*}
then
\begin{equation*}
    \|f(\bm{A})\|_F^2 - \|f(\widehat{\bm{A}}_k)\|_F^2 \leq (1+\varepsilon)\|f(\bm{A})-f(\bm{A}_k)\|_F^2.
\end{equation*}
Then note that
\begin{equation*}
    \|f(\bm{A}) - f(\widehat{\bm{A}}_k)\|_F^2\leq \|f(\bm{A})\|_F^2 - \|f(\widehat{\bm{A}}_k)\|_F^2.
\end{equation*}
It is not entirely black box, since $\|\bm{A}\|_F^2 - \|\widehat{\bm{A}}_k\|_F^2 \leq (1+\varepsilon)\|\bm{A}-\bm{A}_k\|_F^2$ is a stronger condition than $\|\bm{A} -\widehat{\bm{A}}_k\|_F^2 \leq (1+\varepsilon)\|\bm{A}-\bm{A}_k\|_F^2$, but it is at least a start. 

Another thing that you can do is that we know that if $\|(\bm{I}-\bm{P}_{\bm{Q}})\bm{A}\|_F^2 \leq (1+\varepsilon)\|\bm{A}-\bm{A}_k\|_F^2$ then if $\widehat{\bm{A}} = \bm{A} \bm{Q} (\bm{Q}^T \bm{A} \bm{Q})^{\dagger} \bm{Q}^T \bm{A}$ we have
\begin{equation*}
    \|\bm{A}\|_F^2 - \|\widehat{\bm{A}}\|_F^2 \leq \|(\bm{I}-\bm{P}_{\bm{Q}})\bm{A}\|_F^2 \leq (1+\varepsilon)\|\bm{A}-\bm{A}_k\|_F^2
\end{equation*}

\section{Black boxing Schatten norms}
Note that for any operator monotone function $f$ we have
\begin{equation*}
    \|f(\bm{A}) - f(\widehat{\bm{A}}_k)\|_{(p)} \leq \|f(\bm{A}-\widehat{\bm{A}}_k)\|_{(p)}.
\end{equation*}
Let us define $\bm{\Delta} = \bm{A} - \widehat{\bm{A}_k} = \bm{A}^{1/2}(\bm{I} - \bm{P}) \bm{A}^{1/2} = \bm{A}^{1/2} \bm{P}_{\bot} \bm{A}^{1/2}$, where $\bm{P}$ is an orthogonal projection onto a subspace of dimension $k$. 
Suppose that
\begin{equation*}
    \|\bm{\Delta}\|_{(p)} \leq C\|\bm{\Lambda}_2\|_{(p)},
\end{equation*}
for some constant $C \geq 1$. We wish to show that
\begin{equation*}
    \|f(\bm{\Delta})\|_{(p)} \leq C\|f(\bm{\Lambda}_2)\|_{(p)},
\end{equation*}
It is sufficient to show that
\begin{equation*}
    \frac{\|f(\bm{\Delta})\|_{(p)}}{\|f(\bm{\Lambda}_2)\|_{(p)}} \leq \frac{\|\bm{\Delta}\|_{(p)}}{\|\bm{\Lambda}_2\|_{(p)}}.
\end{equation*}
Let $s_i$ be the eigenvalues of $\bm{\Delta}$. By the interlacing theorem we know that $\lambda_{k+j} \leq s_j$.\footnote{The interlacing theorem: Let $\bm{Q} \in \mathbb{R}^{n \times m}$, where $m \leq n$, have orthonormal columns. Let $\bm{B} = \bm{Q}^T \bm{A} \bm{Q}$ where $\bm{A}$ symmetric. Let $\alpha_1 \leq \alpha_2 \leq \cdots \leq \alpha_n$ be the eigenvalues of $\bm{A}$ and $\beta_1 \leq \cdots \beta_m$ be the eigenvalue of $\bm{B}$. Then for $j \leq m$ we have $\alpha_j \leq \beta_j$. We are interested in the case when $m = n-k$ and $\bm{Q}$ is an orthonormal basis for $\range(\bm{P}_{\bot})$. Note that $\alpha_j = \lambda_{n+1-j}$ and $\beta_j = s_{n-k+1-j}$. So for $j \leq n-k$ we have $\lambda_{n+1-j}\leq s_{n-k+1-j}$. Let $\ell = n-j+1$. So for $\ell \geq k+1$ we have $\lambda_{\ell }\leq s_{\ell -k}$. Let $\ell = k + i$. So for $i \geq 1$ we have $\lambda_{k+i} \leq s_i$ as required.} \David{I am not sure if this statement is true. Suppose that the eigenvalues of $\bm{\Delta}$ are $s_1 = 0.86, s_2 = 0.25, s_3 = 0.02$ and the eigenvalues of $\bm{\Lambda}_2$ are $\lambda_{k+1} = 0.86, \lambda_{k+2} = 0.009, \lambda_{k+3} = 0.006$. Then if $f(x) = \sqrt{x}$ we have $\|f(\bm{\Delta})\|_F/\|f(\bm{\Lambda}_2)\|_F \approx 1.14$ but $\|\bm{\Delta}\|_F/\|\bm{\Lambda}_2\|_F \approx 1.04$. I also tried it numerically for real Nystrom approximations, and it is not true. But I have not found a counter example to the black box argument yet, only that this approach cannot help us prove it. }%Hence, since $f(x)/x$ is decreasing we have
%\begin{align*}
    %&\frac{\lambda_{k+j}}{s_i} \leq \frac{f(\lambda_{k+j})}{f(s_i)}\\
    %\Rightarrow & \frac{\lambda_{k+j}^p}{s_i^p} \leq \frac{f(\lambda_{k+j})^p}{f(s_i)^p}\\
    %\Rightarrow & \frac{\|\bm{\Lambda}_2\|_{(p)}^p}{s_i^p} \leq \frac{\|f(\bm{\Lambda}_2)\|_{(p)}^p}{f(s_i)^p}\\
    %\Rightarrow & \frac{s_i^p}{\|\bm{\Lambda}_2\|_{(p)}^p} \geq \frac{f(s_i)^p}{\|f(\bm{\Lambda}_2)\|_{(p)}^p}\\
    %\Rightarrow & \frac{\|\bm{\Delta}\|_{(p)}^p}{\|\bm{\Lambda}_2\|_{(p)}^p} \geq \frac{\|f(\bm{\Delta})\|_{(p)}^p}{\|f(\bm{\Lambda}_2)\|_{(p)}^p}\\
    %\Rightarrow & \frac{\|\bm{\Delta}\|_{(p)}}{\|\bm{\Lambda}_2\|_{(p)}} \geq \frac{\|f(\bm{\Delta})\|_{(p)}}{\|f(\bm{\Lambda}_2)\|_{(p)}}\\
%\end{align*}
%which yields the desired inequality. 


\section{Maybe interesting facts}
Maybe interesting fact: Subspace iteration yields a monotonically better low rank approximation and Nystrom is sandwiched between two iterations of subspace iteration (one sided projections): $\bm{A}$ is spsd.
\begin{align*}
    &\|(\bm{I}-\bm{P}_{\bm{A}^{q}\bm{\Omega}})\bm{A}\|_F^2 \leq \|\bm{A} - \bm{P}_{\bm{A}^{q}\bm{\Omega}}\bm{A}\bm{P}_{\bm{A}^{q}\bm{\Omega}}\|_F^2 \leq \|\bm{A} - \bm{A}^q\bm{\Omega}(\bm{\Omega}^T \bm{A}^{2q-1} \bm{\Omega})^{-1}\bm{\Omega}^T \bm{A}^q\|_F^2 = \\
    & \|\bm{A}^{1/2}(\bm{I}-\bm{P}_{\bm{A}^{q-1/2} \bm{\Omega}})\bm{A}^{1/2}\|_F^2 = \|(\bm{I}-\bm{P}_{\bm{A}^{q-1/2} \bm{\Omega}}) \bm{A}(\bm{I}-\bm{P}_{\bm{A}^{q-1/2} \bm{\Omega}})\|_F^2 \leq \|(\bm{I}-\bm{P}_{\bm{A}^{q-1/2} \bm{\Omega}}) \bm{A}\|_F^2,
\end{align*}
where the first inequality is due to the fact that $\bm{P}_{\bm{A}^{q}\bm{\Omega}})\bm{A}$ minimizes the error over all matrices whose range fall in $\range(\bm{A}^{q}\bm{\Omega})$, the second inequality is due to $\bm{P}_{\bm{A}^{q}\bm{\Omega}})\bm{A}\bm{P}_{\bm{A}^{q}\bm{\Omega}})$ minimizes the error over all matrices whose range and corange falls in $\range(\bm{A}^q\bm{\Omega})$. 








==> interesting_stuff.tex <==
\section{Interestin stuff}
This section contains stuff that we removed, but may still be useful. 

\begin{lemma}
    There exists an orthonormal basis $\bm{V}$ with at most $k$ columns and so that $\range(\bm{V}) \subseteq \range(\bm{Q})$ and 
    \begin{equation*}
        \min\limits_{\bm{C}:\rank(\bm{C}) \leq k} \|\bm{B} - \bm{Q} \bm{C}\|_2 = \|(\bm{I} - \bm{V}\bm{V}^T) \bm{B}\|_2
    \end{equation*}
\end{lemma}
\begin{proof}
Let $\bm{C}_*$ be the optimizer. Let $\bm{V}$ be an orthonormal basis for $\bm{Q}\bm{C}_*$. Since $\bm{C}_*$ is the optimizer we know that
\begin{equation*}
    \|\bm{B} - \bm{Q}\bm{C}_*\|_2 \leq \|(\bm{I} - \bm{V}\bm{V}^T)\bm{B}\|_2.
\end{equation*}
However, we also know by \cite[Lemma 4.14]{woodruff_sketching}
\begin{equation*}
    \min\limits_{\bm{C}}\| \bm{B} - \bm{V} \bm{C}\|_2 = \|(\bm{I}-\bm{V}\bm{V}^T)\bm{B}\|_2.
\end{equation*}
Since we can write $\bm{Q} \bm{C}_* = \bm{V} \widetilde{\bm{C}}_*$ we know that
\begin{equation*}
    \|(\bm{I}-\bm{V}\bm{V}^T)\bm{B}\|_2 \leq \|\bm{B}-\bm{Q} \bm{C}_*\|_2.
\end{equation*}
Consequently,
\begin{equation*}
    \min\limits_{\bm{C}:\rank(\bm{C}) \leq k} \|\bm{B} - \bm{Q} \bm{C}\|_2 = \|(\bm{I} - \bm{V}\bm{V}^T) \bm{B}\|_2,
\end{equation*}
as required. 
\end{proof}

\begin{lemma}
    For any matrix $\bm{B}$ we have
    \begin{equation*}
        \min\limits_{\bm{C} : \rank(\bm{C}) \leq k} \|\bm{B} - \bm{B} \bm{Q} \bm{C}\|_2 \leq \min\limits_{\bm{C} : \rank(\bm{C}) \leq k} \|\bm{B} - \bm{Q} \bm{C}\|_2.
    \end{equation*}
\end{lemma}
\begin{proof}
    We know that $\|(\bm{I} -\bm{P}_{\bm{B} \bm{Q}})\bm{B}\|_2 \leq \|(\bm{I} -\bm{P}_{\bm{Q}})\bm{B}\|_2$. Hence, by \cite[Corollary 5]{kacham2021reduced} we have
\begin{align*}
     &\min\limits_{\bm{C} : \rank(\bm{C}) \leq k} \|\bm{B} - \bm{B} \bm{Q} \bm{C}\|_2 = \max\{\lambda_{k+1},\|(\bm{I}-\bm{P}_{\bm{B} \bm{Q}}) \bm{B}\|_2\} \leq \\
     &\max\{\lambda_{k+1},\|(\bm{I}-\bm{P}_{\bm{Q}}) \bm{B}\|_2\} = \min\limits_{\bm{C} : \rank(\bm{C}) \leq k} \|\bm{B} - \bm{Q} \bm{C}\|_2,
\end{align*}
as required. 
\end{proof}

\David{I think it would be worth checking what the counter examples to "best rank $k$ approximation to $\bm{A}$ whose range is contained in $\bm{Q}$ is not the best rank $k$ approximation of $\bm{Q} \bm{Q}^T \bm{A}$" are. Can we say something additional if we know that $\range(\bm{Q}) \subseteq \range(\bm{A})$? } 

\David{No, numerically this is not true. Even if $\range(\bm{Q}) \subseteq \range(\bm{A})$ the best rank $k$ approximation to $\bm{Q}\bm{Q}^T\bm{A}$ is not optimal}

\David{Another question to ask is if $\|\bm{A} - (\bm{Q} \bm{Q}^T\bm{A})_{(k)}\|_2$ is an increasing function of $\|\bm{A} - \bm{Q} \bm{Q}^T\bm{A}\|_2$ if $k$ is fixed. We know that $\min\limits_{\rank(\bm{X})}\|\bm{A} - \bm{Q} \bm{X}\|_2$ is. }
